Phenomenology of supersymmetric neutrino mass models

The origin of neutrino masses is currently one of the most intriguing questions of particle physics and many extensions of the Standard Model have been proposed in that direction. This experimental evidence is a very robust indication of new physics, but is not the only reason to go beyond the Standard Model. The existence of some theoretical issues supports the idea of a wider framework, supersymmetry being the most popular one. In this thesis, several supersymmetric neutrino mass models have been studied. In the first part, the phenomenology of models with bilinear-like R-parity violation is discussed in great detail, highlighting the most distinctive signatures at colliders and low energy experiments. In particular, the correlations between the LSP decay and neutrino physics are shown to be a powerful tool to put this family of models under experimental test. Other important signatures are investigated as well, like majoron emission in charged lepton decays for the case of models with spontaneous breaking of R-parity. A very different approach is followed in the second part of the thesis. Supersymmetric models with a Left-Right symmetry have all the ingredients to incorporate a type-I seesaw mechanism for neutrino masses and conserve R-parity at low energies. In this case, which only allows for indirect tests, the generation of neutrino masses at the high seesaw scale is encoded at low energies in the slepton soft masses. Contrary to minimal seesaw models, sizeable flavor violation in the right slepton sector is expected. Its experimental observation would be a clear hint of an underlying Left-Right symmetry, providing valuable information about physics at very high energies.

==> Intro_sp.tex <==

\section{Introducci\'on}

La investigaci\'on desarrollada en esta tesis doctoral tiene como objetivo la caracterizaci\'on de la masa del neutrino en teor\'ias supersim\'etricas, tanto en modelos a baja como alta escala, y el estudio de la fenomenolog\'ia resultante en colisionadores (como el LHC o un futuro ILC), f\'isica de astropart\'iculas y cosmolog\'ia.

El hist\'orico descubrimiento de las oscilaciones del neutrino marc\'o un momento crucial en la f\'isica de part\'iculas e implica que los neutrinos tienen masa. \'Este es hoy en d\'ia un activo campo de investigaci\'on que trata las interdependencias entre la f\'isica de part\'iculas, nuclear, astrof\'isica y cosmolog\'ia, \'areas en las que el neutrino juega un papel central.

Gracias a la precisi\'on adquirida por los experimentos m\'as modernos ha sido posible determinar los valores de los par\'ametros que intervienen en las oscilaciones de sabor observadas en diversos experimentos, obteni\'endose una concordancia total y conduciendo a la aceptaci\'on del mecanismo oscilatorio como el causante del fen\'omeno observado. Por ello, debido a la ausencia de las masas de los neutrinos en el Modelo Est\'andar de la f\'isica de part\'iculas, se ha hecho necesario ir m\'as all\'a de los marcos te\'oricos establecidos para explicar su origen.

Por otro lado, el Modelo Est\'andar presenta tambi\'en ciertos problemas te\'oricos que nos hacen pensar que es una teor\'ia incompleta. En particular, la sensibilidad de la masa del bos\'on de Higgs a la existencia de part\'iculas pesadas requiere un ajuste muy fino de los par\'ametros para que la masa de dicha part\'icula se encuentre a la escala electrod\'ebil. Este problema de naturalidad se conoce como problema de la jerarqu\'ia. Muchas ideas han sido desarrolladas con el objetivo de solucionar este defecto del Modelo Est\'andar. La m\'as popular de ellas, Supersimetr\'ia, proporciona una soluci\'on t\'ecnica al problema de la jerarqu\'ia, al tiempo que cuenta con los ingredientes necesarios para acomodar nueva f\'isica. En el caso de los neutrinos, una simetr\'ia discreta, llamada Paridad R y definida como $R_p = (-1)^{3(B-L)+2s}$, con $B$ y $L$ los n\'umeros bari\'onico y lept\'onico y $s$ el esp\'in de la part\'icula, juega un papel determinante. Tanto el origen de esta simetr\'ia como su conexi\'on con la generaci\'on de masa de los neutrinos son temas que merecen ser investigados en profundidad.

La presente tesis puede dividirse en dos l\'ineas de investigaci\'on \'intimamente ligadas entre s\'i. Por un lado, se ha estudiado en detalle la fenomenolog\'ia de modelos supersim\'etricos de masa de neutrinos con violaci\'on de Paridad R. Este tipo de teor\'ias ofrece una fenomenolog\'ia muy rica en los experimentos presentes o del futuro pr\'oximo. Por lo tanto, el estudio de las se\~nales experimentales previstas es fundamental para entender la conexi\'on entre la teor\'ia subyacente y los datos obtenidos por las colaboraciones experimentales. Por otro lado, se ha abordado tambi\'en la situaci\'on opuesta. Si Paridad R se conserva, la masa de los neutrinos debe generarse de otro modo. Esto nos ha llevado a estudiar cu\'al es el origen de Paridad R y c\'omo puede estar relacionado con la masa de los neutrinos. En concreto, las teor\'ias supersim\'etricas con simetr\'ia Left-Right representan un marco ideal para ello, pues pueden dar lugar a conservaci\'on de Paridad R a bajas energ\'ias e incorporan el mecanismo seesaw para generar la masa de los neutrinos.

Finalmente, no debemos olvidar que estamos viviendo un momento de gran expectaci\'on en la f\'isica de part\'iculas, debido a la reciente puesta en marcha del LHC. Esto pronto provocar\'a la llegada de abundantes datos experimentales con una muy valiosa informaci\'on sobre los componentes fundamentales de la materia. Por lo tanto, esta tesis se centra principalmente en cuestiones fenomenol\'ogicas, concentr\'andose en el LHC y otros experimentos que intentar\'an desentra\~nar los misterios que la naturaleza todav\'ia nos oculta.

\section{Motivaci\'on}

La invenci\'on del Modelo Est\'andar a principios de los a\~nos 70 del pasado siglo puede considerarse el \'ultimo gran hito de la f\'isica de part\'iculas\footnote{Se recomienda la lectura de la referencia \cite{Weinberg:2004kv}, donde uno de los padres del Modelo Est\'andar narra sus impresiones y describe la creaci\'on de la teor\'ia desde un punto de vista hist\'orico.}. Esta perfecta combinaci\'on de diversas ideas te\'oricas, acopladas de la forma precisa para describir los fen\'omenos observados, sigue siendo a d\'ia de hoy uno de los pilares fundamentales sobre los que se apoya nuestro entendimiento del mundo que nos rodea.

De hecho, a lo largo de los a\~nos numerosos experimentos lo han puesto a prueba obteniendo, salvo en las contadas ocasiones que mencionaremos m\'as adelante, un acuerdo espectacular con las predicciones te\'oricas. Por lo tanto, podemos afirmar sin lugar a dudas que el Modelo Est\'andar describe con una alt\'isima precisi\'on el mundo de las part\'iculas fundamentales\footnote{No obstante, no debemos olvidar que, de todas las part\'iculas predichas por el Modelo Est\'andar, todav\'ia hay una que est\'a por descubrir. El bos\'on de Higgs, el rastro dejado tras la rotura espont\'anea de la simetr\'ia electrod\'ebil, es objeto de intensa b\'usqueda experimental en numerosos experimentos actuales.}.

Tal es la concordancia entre el Modelo Est\'andar y los resultados experimentales obtenidos en los \'ultimos a\~nos que cualquier extensi\'on, por m\'inima que sea, est\'a fuertemente acotada. En cierto modo, el Modelo Est\'andar se ha convertido en un punto de partida indispensable para cualquier intento te\'orico de explicar las interacciones a nivel subat\'omico y cualquier teor\'ia extendida debe ser capaz de obtener el Modelo Est\'andar como su l\'imite de bajas energ\'ias. 

No obstante, y pese al \'exito ya mencionado, el Modelo Est\'andar cuenta hoy en d\'ia con ciertos problemas que nos hacen pensar que no es \emph{la teor\'ia definitiva}, sino otro paso m\'as hacia una imagen mucho m\'as amplia. Estas indicaciones de f\'isica m\'as all\'a del Modelo Est\'andar pueden clasificarse principalmente en:

\begin{itemize}
\item Problemas te\'oricos
\end{itemize}

El Modelo Est\'andar da lugar a ciertas dificultades a la hora de entender algunos de sus detalles, lo que ha motivado una intensa b\'usqueda de extensiones con el objetivo de dotarle de solidez te\'orica. De entre todos estos problemas destacaremos uno en especial, dada su importancia para el desarrollo de esta tesis: el problema de la jerarqu\'ia.

Por un lado, existen poderosas razones para pensar que el Modelo Est\'andar no es la \'ultima palabra en f\'isica de part\'iculas. Entre otros motivos, hoy en d\'ia no contamos con una teor\'ia cu\'antica de la gravedad que sea capaz de extender la Relatividad General de Einstein al mundo de lo microsc\'opico. Por ello, esperamos que un nuevo paradigma f\'isico, una nueva estructura te\'orica todav\'ia no concebida, aparezca a escalas de energ\'ias pr\'oximas a la escala de Planck, $M_P = 10^{18}$ GeV, donde los efectos cu\'anticos de la gravedad comienzan a ser relevantes.

Del mismo modo, tambi\'en se especula sobre la existencia de otras escalas intermedias entra la escala de Planck y la escala electrod\'ebil. Por ejemplo, la escala a la que se unifican los acoplamientos gauge, o escala de gran unificaci\'on, se situar\'ia en torno a los $10^{16}$ GeV, tal y como se deduce de consideraciones te\'oricas y fenomenol\'ogicas\footnote{Este n\'umero debe tomarse a t\'itulo ilustrativo. Modelos determinados pueden predecir escalas de gran unificaci\'on diferentes.}. Otra escala intermedia podr\'ia ser la escala a la que se genera la masa de los neutrinos o, similarmente, la escala a la que una determinada teor\'ia de sabor capaz de explicar las masas de los fermiones resulte efectiva. En todos estos casos habr\'ia que extender el Modelo Est\'andar y a\~nadir nuevas part\'iculas pesadas, responsables de la f\'isica a altas energ\'ias.

Por otro lado, a esto cabe a\~nadir la bien conocida sensibilidad del bos\'on de Higgs\footnote{De hecho, este problema est\'a asociado a cualquier part\'icula escalar, aunque resulte especialmente alarmante en el caso del bos\'on de Higgs, pues la fenomenolog\'ia requiere que su masa se encuentre a la escala electrod\'ebil.}, una pieza esencial del Modelo Est\'andar, a la existencia de escalas de energ\'ias m\'as altas. Al valor de su masa al nivel \'arbol se deben a\~nadir las diversas correcciones radiativas procedentes de sus interacciones con otras part\'iculas y, dado que el bos\'on de Higgs se acopla al resto de part\'iculas proporcionalmente a sus masas, part\'iculas m\'as pesadas dan lugar a correcciones m\'as grandes. De hecho, un c\'alculo expl\'icito muestra que la masa del bos\'on de Higgs, $m_h$, recibe correciones de la forma

\begin{equation}
\Delta m_h^2 \propto \Lambda^2
\end{equation}

siendo $\Lambda$ la escala a la que se encuentra la nueva f\'isica. Por ejemplo, $\Lambda$ puede ser la masa de una part\'icula superpesada a escalas cercanas a la escala de Planck.

Estas divergencias cuadr\'aticas, as\'i llamadas por ser proporcionales al cuadrado de la nueva escala de energ\'ias, son generadas por todas las part\'iculas que puedan interaccionar con el bos\'on de Higgs. Por lo tanto, uno finalmente obtiene 

\begin{equation}
m_h^2 = (m_h)_0^2 + (\Delta m_h^2)_1 + (\Delta m_h^2)_2 + \dots
\end{equation}

Tras sumar todas las contribuciones al valor de nivel \'arbol, $(m_h)_0$, uno debe obtener una masa $m_h$ en la escala electrod\'ebil. En caso contrario, la rotura espont\'anea de la simetr\'ia, principal motivaci\'on para incluir el bos\'on de Higgs en la teor\'ia, dejar\'ia de funcionar. Por lo tanto, cantidades que pueden llegar a valores del orden de $\pm (10^{18}$ GeV$)^2$ deben sumarse entre s\'i para dar lugar a un resultado final que se encuentre alrededor de $(100$ GeV$)^2$. 

Aunque esto es perfectamente consistente desde un punto de vista estrictamente te\'orico, resulta sorprendente que el Modelo Est\'andar precise tal \emph{coincidencia} para dar lugar a la f\'isica que conocemos. Por ello, el fort\'isimo ajuste fino de los par\'ametros necesario a cada orden en teor\'ia de perturbaciones para estabilizar la masa del bos\'on de Higgs y situarla en la escala electrod\'ebil est\'a considerado por la gran mayor\'ia de los te\'oricos como un problema de naturalidad, el famoso problema de la jerarqu\'ia.

Podr\'iamos mencionar otros detalles te\'oricos no completamente comprendidos en el Modelo Est\'andar, como el origen de la rotura espont\'anea de la simetr\'ia electrod\'ebil, la posible unificaci\'on de los acoplamientos gauge o la replicaci\'on en familias de quarks y leptones. Todos ellos han dado lugar a numerosas ideas especulativas sobre extensiones del Modelo Est\'andar, algunas de las cuales ser\'an mencionadas en esta tesis.

\begin{itemize}
\item Problemas experimentales
\end{itemize}

Adem\'as de los problemas te\'oricos ya mencionados el Modelo Est\'andar cuenta tambi\'en con ciertas discrepancias con resultados experimentales. As\'i como los primeros se basan en nuestra interpretaci\'on, no siempre libre de prejuicios te\'oricos, estos problemas son indudables y requieren la adici\'on de nuevos elementos que puedan darles soluci\'on.

La m\'as patente de todas las discrepancias observadas es el reciente descubrimiento de la masa de los neutrinos \cite{Ahmad:2002jz,Fukuda:1998mi,Eguchi:2002dm,kl:2008ee,Hosaka:2006zd,Adamson:2008zt}, uno de los puntos de partida de la presente tesis.

Motivados por la observaci\'on emp\'irica de que todos los neutrinos presentan quiralidad izquierda en los experimentos realizados, los padres del Modelo Est\'andar no a\~nadieron neutrinos de quiralidad derecha al espectro de la teor\'ia. Esta decisi\'on, que adem\'as va en la sensata direcci\'on de a\~nadir el m\'inimo n\'umero de ingredientes, provoca que los neutrinos no adquiran masa en el Modelo Est\'andar\footnote{Este hecho no se limita al nivel \'arbol. Puede comprobarse que la simetr\'ia global $U(1)_{B-L}$ del Modelo Est\'andar garantiza que los neutrinos no adquieran masa a ning\'un orden en teor\'ia de perturbaciones. No obstante, es posible generar masas de neutrinos sin necesidad de a\~nadir neutrinos dextr\'ogiros simplemente rompiendo dicha simetr\'ia mediante la adici\'on de otras nuevas part\'iculas, tal y como se muestra en el cap\'itulo \ref{chap:numass} de esta tesis.}.

Durante muchos a\~nos esta hip\'otesis result\'o v\'alida, pues todos los experimentos que intentaron encontrar una desviaci\'on respecto de $m_\nu = 0$ fueron incapaces de observar se\~nal alguna. Sin embargo, la existencia de ciertas anomal\'ias asociadas a los neutrinos, los llamados problemas de los neutrinos solares y atmosf\'ericos, perturbaron esta calma.

La f\'isica nuclear y su correspondiente aplicaci\'on en astrof\'isica estelar han dado como resultado un buen conocimiento de los mecanismos de producci\'on de neutrinos en el interior del Sol. De ese modo, gracias al llamado Modelo Solar Est\'andar\footnote{Para detalles sobre el Modelo Solar Est\'andar y el flujo de neutrinos solares v\'ease por ejemplo \cite{Bahcall:2004pz} y las referencias que en este art\'iculo se encuentran.}, uno puede predecir con cierta precisi\'on el flujo de neutrinos que esperamos recibir en la Tierra. Estos resultados te\'oricos, robustos y bien comprendidos, han sido sin embargo desafiados en numerosas ocasiones por los experimentos. Diversas colaboraciones han dedicado su esfuerzo a detectar los neutrinos procedentes del Sol, obteniendo siempre un n\'umero menor al esperado \cite{Davis:1994jw}. A esta anomal\'ia se la conoce como ``Problema de los neutrinos solares''.

Del mismo modo, otra anomal\'ia ha sido observada en la detecci\'on de los neutrinos atmosf\'ericos. \'Estos son producidos cuando los rayos c\'osmicos colisionan con las mol\'eculas de las capas superiores de nuestra atm\'osfera. Las part\'iculas producidas en el choque viajan hacia la Tierra, desintegr\'andose y dando lugar a neutrinos, entre otros productos. Es posible estimar el n\'umero de neutrinos esperado en la superficie, a trav\'es de simulaciones con m\'etodos de Monte Carlo \cite{Gaisser:1988ar,Barr:1989ru,Honda:2004yz}, y comparar con los neutrinos observados. De nuevo, el resultado obtenido ha sido bien diferente del esperado. En particular, aunque se esperaba que el cociente $R_{e \mu} \equiv N(\nu_\mu)/N(\nu_e)$ entre el n\'umero de neutrinos mu\'onicos y electr\'onicos detectados fuera cercano a $2$, se observ\'o un cociente $0.6$ veces menor, v\'ease por ejemplo \cite{Fukuda:1996sz}. A esta anomal\'ia se la conoce como ``Problema de los neutrinos atmosf\'ericos''.

Tras a\~nos de investigaci\'on experimental, la llegada de datos procedentes de experimentos con neutrinos atmosf\'ericos y de reactor ha servido para determinar finalmente la soluci\'on a estos d\'eficits. \'Esta est\'a basada en el mecanismo de las oscilaciones de neutrinos \cite{Pontecorvo:1967fh}, seg\'un el cual los neutrinos, producidos como autoestados de sabor, evolucionan en su propagaci\'on oscilando de un sabor a otro. Esto explicar\'ia la aparente desaparici\'on de los neutrinos observada en diferentes experimentos. Ahora bien, para que las oscilaciones de neutrinos sean posibles es necesario que tengan masa.

Por lo tanto, el descubrimiento de las oscilaciones de los neutrinos supuso un momento crucial en la f\'isica de part\'iculas por implicar que los neutrinos tienen masa no nula. Esto a su vez significa que el Modelo Est\'andar debe extenderse para incorporar un mecanismo que genere dicha masas.

Como nota final a\~nadamos que existen otros resultados experimentales que el Modelo Est\'andar no puede acomodar. El m\'as s\'olido de estos indicios de nueva f\'isica es la materia oscura del universo \cite{Komatsu:2010fb}, para la cual no hay candidato alguno entre las part\'iculas conocidas. Del mismo modo, otra observaci\'on cosmol\'ogica, en este caso la llamada asimetr\'ia bari\'onica del universo, es otro reto para los te\'oricos actuales. Ambas son buenas raz\'ones para ir m\'as all\'a del Modelo Est\'andar.\\

A lo largo de esta tesis se han abordado ambos tipos de problemas del Modelo Est\'andar, tanto te\'oricos como experimentales, proponiendo soluciones a ambos y describiendo qu\'e se\~nales experimentales se esperan si las extensiones propuestas son las escogidas por la naturaleza.

\section{El Modelo Est\'andar y Supersimetr\'ia}

Comenzaremos la discusi\'on describiendo brevemente los conceptos fundamentales tras el Modelo Est\'andar, c\'omo aparece el problema de la jerarqu\'ia y qu\'e soluci\'on ofrece Supersimetr\'ia. En el cap\'itulo \ref{chap:susy} se profundiza en estos temas, ofreciendo adem\'as numerosas referencias a los textos apropiados para una introducci\'on m\'as completa.

El Modelo Est\'andar es una teor\'ia gauge basada en el grupo $SU(3)_c \times SU(2)_L \times U(1)_Y$. Una vez fijado el grupo de gauge queda determinado el contenido de part\'iculas de esp\'in 1, es decir, los bosones de gauge del modelo. En concreto, hay 8 bosones de gauge para $SU(3)_c$, los gluones, 3 para $SU(2)_L$, los bosones W, y 1 para el grupo $U(1)_Y$, el bos\'on B.

\begin{figure}
\begin{center}
\vspace{5mm}
\includegraphics[width=0.5\textwidth]{img/Higgs.eps}
\end{center}
\vspace{0mm}
\caption{El bos\'on de Higgs es la \'ultima pieza que cada por descubrir en el Modelo Est\'andar. Propuesto por Peter Higgs a mediados de los a\~nos 60, es el rastro dejado por el mecanismo de rotura espont\'anea de la simetr\'ia. Sin lugar a dudas, es el objetivo principal en la b\'usqueda del colisionador LHC.}
\label{fig:higgs-intro}
\end{figure}

Los fermiones deben ser asignados a representaciones irreducibles del grupo de gauge. Por un lado, la pieza $SU(2)_L \times U(1)_Y$ describe las interacciones d\'ebiles y electromagn\'eticas. Mientras que los fermiones de quiralidad izquierda se colocan en dobletes de $SU(2)_L$, los de quiralidad derecha son singletes, y por lo tanto no se acoplan a los correspondientes bosones de gauge. De este modo se introduce expl\'icitamente en la teor\'ia la violaci\'on de paridad observada experimentalmente en las interacciones d\'ebiles. Por otro lado, la pieza $SU(3)_c$ es la responsable de las interacciones fuertes que sienten los quarks, y por lo tanto \'estos son colocados en tripletes de este subgrupo.

\begin{table}
\begin{center}
{
\renewcommand\arraystretch{1.5} %(1.0 is for standard spacing)
\begin{tabular}{|c|c|c|c|c|}
\hline
Nombre & Representaci\'on & $SU(3)_c$, $SU(2)_L$, $U(1)_Y$ \\
\hline
\hline
\multirow{3}{*}{quarks} &  ($u_L$ $d_L$) & ( 3 , 2 , $\frac{1}{6}$ )\\
& $u_R^c$ & ( 3 , 1 , $-\frac{2}{3}$ )\\
& $d_R^c$ & ( 3 , 1 , $\frac{1}{3}$ )\\
\hline
\multirow{2}{*}{leptones} &  ($\nu_L$ $l_L$) & ( 1 , 2 , $-\frac{1}{2}$ )\\
& $l_R^c$ & ( 1 , 1 , 1 )\\
\hline
\hline
Higgs & ($\phi^+$ $\phi^0$) & ( 1 , 2 , $\frac{1}{2}$ )\\
\hline
\hline
bos\'on B & $B^0$ & ( 1 , 1 , 0 )\\
\hline
bosones W & $W_1$, $W_2$, $W_3$ & ( 1 , 3 , 0 )\\
\hline
gluones & $g$ & ( 8 , 1 , 0 )\\
\hline
\end{tabular}
}
\end{center}
\caption[SM particle content Intro]{Contenido de part\'iculas del Modelo Est\'andar. La hipercarga se define siguiendo la convenci\'on $Q = I_{3L}+Y$. Solamente se presenta la primera familia de quarks y leptones.} \label{sm-particle-content-intro}
\end{table}

Finalmente, es un hecho bien conocido que en teor\'ias de Yang-Mills no est\'a permitido escribir t\'erminos de masa para las reprentaciones no singlete. Esto viene impuesto por la propia simetr\'ia gauge. Por lo tanto, la simetr\'ia debe romperse de alg\'un modo para generar las masas de los fermiones y los bosones de gauge. Esto se hace mediante la inclusi\'on de un doblete de $SU(2)_L$, el cual adquiere un valor de expectaci\'on en el vac\'io (VEV) rompiendo la simetr\'ia electrod\'ebil de forma espont\'anea. El grupo de simetr\'ia resultante tras este proceso es $SU(3)_c \times U(1)_Q$, donde $Q$ es la carga el\'ectrica. Adem\'as, una de las componentes reales del doblete permanece en el espectro como una part\'icula f\'isica, el c\'elebre bos\'on de Higgs.

En la tabla \ref{sm-particle-content-intro} se muestra el contenido de part\'iculas del Modelo Est\'andar. N\'otese que la \'unica part\'icula no descubierta de entre todas ellas es el bos\'on de Higgs, principal objetivo de la b\'usqueda llevada a cabo en los colisionadores presentes, sobre el que hablaremos a continuaci\'on.

Sea $H$ el doblete de Higgs introducido para romper la simetr\'ia electrod\'ebil. Es com\'un denotarlo de la siguiente forma

\begin{equation}
H = \left( \begin{array}{c}
\phi^+ \\
\phi^0 \end{array} \right)
\end{equation}

N\'otese que, usando la convenci\'on $Q = I_{3L} + Y$, $H$ tiene hipercarga $Y=+\frac{1}{2}$. Con estos ingredientes el potencial escalar m\'as general invariante bajo el grupo de gauge es

\begin{equation} \label{pot-intro}
V(H^\dagger H) = \mu^2 H^\dagger H + \lambda (H^\dagger H)^2
\end{equation}

donde $\mu$ es un par\'ametro con dimensiones de masa y $\lambda$ un acoplamiento sin dimensiones. El an\'alisis de este potencial revela que $\mu^2 < 0$ es una condici\'on necesaria para que el m\'inimo del potencial no se encuentre en $H = 0$ y pueda as\'i romperse la simetr\'ia. En ese caso la componente neutra de $H$, $\phi^0$, adquiere un VEV no nulo $\langle \phi^0 \rangle = \frac{v}{\sqrt{2}}$, donde

\begin{equation}
v = \sqrt{-\frac{\mu^2}{\lambda}}
\end{equation}

y el campo $\phi^0$ puede reescribirse respecto a su VEV como

\begin{equation}
\phi^0 = \frac{h+v}{\sqrt{2}}
\end{equation}

Adem\'as, de las expresiones anteriores es inmediato obtener que la masa del bos\'on de Higgs, $h$, el estado f\'isico resultante tras la rotura espont\'anea de $SU(2)_L \times U(1)_Y$, es $m_h = \sqrt{-2 \mu^2}$.

No obstante, no olvidemos que dicho valor se corresponde con la masa a nivel \'arbol. A esto cabe a\~nadir correcciones radiativas que, como veremos, pueden modificar sensiblemente el valor original. Por ejemplo, consideremos un escalar $S$ con masa $m_S$ que tiene un t\'ermino de interacci\'on con el Higgs de la forma $- \lambda_S |H|^2 |S|^2$. Es sencillo calcular la correcci\'on a 1-loop que este nuevo t\'ermino generar\'ia para la masa del bos\'on de Higgs:

\begin{equation}
\left( \Delta m_h^2 \right)_S \sim \lambda_S \int \frac{d^4p}{(2 \pi)^4} \frac{1}{p^2-m_S^2}
\end{equation}

Del mismo modo, si consideramos un acoplamiento a un fermi\'on $f$ de masa $m_f$ que se acopla al bos\'on de Higgs con un t\'ermino $- \lambda_f H \bar{f} P_L f + h.c.$, donde $P_L = \frac{1}{2}(1-\gamma_5)$ es el proyector de quiralidad izquierda, obtenemos una correci\'on de la forma

\begin{equation}
\left( \Delta m_h^2 \right)_f \propto - |\lambda_f|^2 \int \frac{d^4p}{(2 \pi)^4} \frac{1}{p^2-m_f^2}
\end{equation}

En ambos casos un simple an\'alisis dimensional nos dice que las correcciones involucran divergencias cuadr\'aticas. Por lo tanto, se puede escribir $\Delta m_h^2 \propto \Lambda^2$, siendo $\Lambda$ la escala de energ\'ias que genera la correcci\'on, dada en estos casos por las masas $m_S$ y $m_f$. Como esperamos la existencia de nueva f\'isica a escalas de energ\'ias muy elevadas, por ejemplo a la escala de Planck ($M_P = 10^{18}$ GeV) con una teor\'ia de gravedad cu\'antica, estas correciones son potencialmente muy grandes.

Ahora, si tenemos en cuenta que tras sumar todas las correcciones debe obtenerse una masa $m_h$ en la escala electrod\'ebil, o de lo contrario la rotura espont\'anea de la simetr\'ia no funcionar\'ia, resulta sorprendente que cantidades que pueden llegar a $\pm (10^{18}$ GeV$)^2$ deban cancelarse entre s\'i de una forma muy precisa a todos los \'ordenes en teor\'a de perturbaciones para dar lugar a un resultado final de alrededor de $(100$ GeV$)^2$. Esto es lo que se conoce como ``Problema de la jerarqu\'ia''\footnote{El lector interesado encontrar\'a una descripci\'on muy pedag\'ogica del problema de la jerarqu\'ia en la referencia \cite{Drees:1996ca}.}.

N\'otese que este ajuste tan fino de los par\'ametros puede evitarse si se dan las condiciones

\begin{eqnarray}
m_S^2 &=& m_f^2 \label{hie-intro-sol1} \\
\lambda_S &=& | \lambda_f |^2 \label{hie-intro-sol2}
\end{eqnarray}

En ese caso las contribuciones a 1-loop del escalar $S$ y el fermi\'on $f$ se cancelan exactamente. Del mismo modo, puede comprobarse que lo mismo sucede con los \'ordenes superiores. No obstante, para que algo as\'i suceda debe haber una raz\'on, una simetr\'ia que lo fuerce. Esa simetr\'ia es Supersimetr\'ia.

Supersimetr\'ia es una simetr\'ia que relaciona bosones y fermiones. Haag, Lopuszanski y Sohnius \cite{Haag:1974qh} mostraron en 1975 que es posible extender las simetr\'ias del espacio-tiempo incluyendo nuevos generadores fermi\'onicos. En lugar de seguir relaciones de conmutaci\'on, los generadores fermi\'onicos obedecen relaciones de anticonmutaci\'on. Esto permite evadir el famoso teorema de Coleman y Mandula \cite{Coleman:1967ad}, y as\'i unificar el grupo de Poincar\'e con las simetr\'ias internas del sistema.

Los generadores de Supersimetr\'ia, $Q_{\alpha}$ y $\bar{Q}_{\dot{\alpha}}$, son espinores de Weyl de dos componentes ($\alpha, \dot{\alpha} = 1, 2$). Su acci\'on sobre los campos transforma fermiones en bosones y viceversa

\begin{equation}
Q_{\alpha} |\text{fermi\'on} \rangle = |\text{bos\'on} \rangle \quad , \quad \bar{Q}_{\dot{\alpha}} |\text{bos\'on} \rangle = | \text{fermi\'on} \rangle
\end{equation}

y por lo tanto las teor\'ias invariantes bajo transformaciones supersim\'etricas deben obedecer unas relaciones como las vistas en las ecuaciones \eqref{hie-intro-sol1} y \eqref{hie-intro-sol2}.

Como vemos, su aparici\'on en la f\'isica de part\'iculas se debi\'o a razones puramente formales. No obstante, la principal motivaci\'on para el estudio de la Supersimetr\'ia en esta tesis es la soluci\'on que proporciona para el problema de la jerarqu\'ia. De hecho, este detalle fue pronto observado, y la extensi\'on m\'inima supersim\'etrica del Modelo Est\'andar (MSSM, por su nombre en ingl\'es, Minimal Supersymmetric Standard Model) fue propuesta en los a\~nos 80 precisamente como una soluci\'on al problema de la jerarqu\'ia \cite{Dimopoulos:1981zb}. Desde entonces ha sido objeto de intenso estudio por parte de numerosos trabajos que han explorado su fenomenolog\'ia e implicaciones experimentales.

\begin{table}
\begin{center}
{
\renewcommand\arraystretch{1.5} %(1.0 is for standard spacing)
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Nombre} & Esp\'in 0 & Esp\'in 1/2 & $SU(3)_c$, $SU(2)_L$, $U(1)_Y$ \\
\hline
\hline
\multirow{3}{*}{squarks, quarks} & $\widehat{Q}$ & ($\tilde{u}_L$ $\tilde{d}_L$) &  ($u_L$ $d_L$) & ( 3 , 2 , $\frac{1}{6}$ )\\
& $\widehat{u}^c$ & $\tilde{u}_R^*$ & $u_R^c$ & ( 3 , 1 , $-\frac{2}{3}$ )\\
& $\widehat{d}^c$ & $\tilde{d}_R^*$ & $d_R^c$ & ( 3 , 1 , $\frac{1}{3}$ )\\
\hline
\multirow{2}{*}{sleptones, leptones} & $\widehat{L}$ & ($\tilde{\nu}_L$ $\tilde{l}_L$) &  ($\nu_L$ $l_L$) & ( 1 , 2 , $-\frac{1}{2}$ )\\
& $\widehat{e}^c$ & $\tilde{l}_R^*$ & $l_R^c$ & ( 1 , 1 , 1 )\\
\hline
\multirow{2}{*}{Higgs, higgsinos} & $\widehat{H}_d$ & ($H_d^0$ $H_d^-$) &  ($\tilde{H}_d^0$ $\tilde{H}_d^-$) & ( 1 , 2 , $-\frac{1}{2}$ )\\
& $\widehat{H}_u$ & ($H_u^+$ $H_u^0$) & ($\tilde{H}_u^+$ $\tilde{H}_u^0$) & ( 1 , 2 , $\frac{1}{2}$ )\\
\hline
\end{tabular}

\vspace{0.4cm}

\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Nombre} & Esp\'in 1/2 & Esp\'in 1 & $SU(3)_c$, $SU(2)_L$, $U(1)_Y$ \\
\hline \hline
bino, bos\'on B & $\widehat{V}_1$ & $\tilde{B}^0$ & $B^0$ & ( 1 , 1 , 0 )\\
\hline
wino, bosones W & $\widehat{V}_2$ & $\tilde{W}_1$, $\tilde{W}_2$, $\tilde{W}_3$ & $W_1$, $W_2$, $W_3$ & ( 1 , 3 , 0 )\\
\hline
gluino, gluones & $\widehat{V}_3$ & $\tilde{g}$ & $g$ & ( 8 , 1 , 0 )\\
\hline
\end{tabular}
}
\end{center}
\caption[MSSM particle content Intro]{Contenido de part\'iculas del MSSM. La hipercarga se define siguiendo la convenci\'on $Q = I_{3L}+Y$. Solamente se presenta la primera familia de quarks y leptones.} \label{mssm-particle-content-intro}
\end{table}

En el MSSM cada part\'icula del Modelo Est\'andar se encuentra en un supermultiplete junto con su supercompa\~nero, lo que da lugar a una duplicaci\'on del contenido de part\'iculas. A esto hay que a\~nadir la necesidad de contar con dos dobletes de Higgs, y no solamente uno, para as\'i dotar de masa simult\'aneamente a los quarks de tipo up y a los quarks de tipo down. Esto se debe a las restricciones que impone Supersimetr\'ia. Adem\'as, la adici\'on de un segundo doblete de Higgs sirve tambi\'en para cancelar las anomal\'ias gauge que aparecen al supersimetrizar el Modelo Est\'andar y a\~nadir nuevos fermiones, los higgsinos en este caso.

El contenido de part\'iculas del MSSM puede consultarse en la tabla \ref{mssm-particle-content-intro}. N\'otese que el grupo de gauge, y las cargas asociadas bajo el mismo, son las mismas que en el Modelo Est\'andar.

A continuaci\'on discutiremos brevemente dos detalles fundamentales del MSSM que requieren cierta atenci\'on por nuestra parte: (1) la rotura soft de Supersimetr\'ia, y (2) la Paridad R.

Si la Supersimetr\'ia existe en la naturaleza, no puede ser una simetr\'ia exacta. De lo contrario, habr\'ia una part\'icula escalar con las misma masa y carga del electr\'on, que deber\'ia haber sido descubierta hace muchos a\~nos. Como no es as\'i, Supersimetr\'ia debe romperse de alg\'un modo.

Aunque hay muchas ideas al respecto, es com\'un parametrizarlas todas ellas en los llamados t\'erminos \emph{soft} \cite{Girardello:1981wz}. Estos t\'erminos se a\~naden al lagrangiano para romper de forma expl\'icita la simetr\'ia entre fermiones y bosones. Por ejemplo, pueden a\~nadirse masas para los escalares, que los distingan claramente de los fermiones.

De este modo se generan diferencias entre las part\'iculas del Modelo Est\'andar y las llamadas superpart\'iculas, sus compa\~neros supersim\'etricos. Podr\'ia parecer que al romper Supersimetr\'ia se pierde su principal motivaci\'on, la soluci\'on al problema de la jerarqu\'ia. No obstante, si los nuevos t\'erminos soft son del orden del TeV, se explicar\'ia la no detecci\'on de las superpart\'iculas en los experimentos realizados, al tiempo que se mantendr\'ia la soluci\'on t\'ecnica al problema de la jerarqu\'ia.

El segundo comentario a realizar est\'a asociado a los n\'umeros bari\'onico (B) y lept\'onico (L). As\'i como en el Modelo Est\'andar ambos se encuentran conservados por accidente, al realizar una extensi\'on supersim\'etrica se encuentran nuevos t\'erminos que rompen estas dos simetr\'ias discretas. Esto se debe esencialmente a la existencia de los squarks y los sleptones, los compa\~neros supersim\'etricos de quarks y leptones, que pueden dar lugar a nuevos v\'ertices que violan B o L.

En concreto, adem\'as de los acoplamientos de Yukawa ya presentes en el Modelo Est\'andar y el t\'ermino de mezcla entre los dos dobletes de Higgs, se obtienen los siguientes t\'erminos en el superpotencial

\begin{equation} \label{rpv-superpotential-intro}
W^{\textnormal{\rpv}} = \frac{1}{2} \lambda_{ijk} \widehat{L}_i \widehat{L}_j \widehat{e^c}_k  + \lambda'_{ijk} \widehat{L}_i \widehat{Q}_j \widehat{d^c}_k + \frac{1}{2} \lambda''_{ijk} \widehat{u^c}_i \widehat{d^c}_j \widehat{d^c}_k + \epsilon_i \widehat{L}_i \widehat{H}_u
\end{equation}

Como estas interacciones no han sido observadas jam\'as en la naturaleza y dado que la existencia simult\'anea de violaci\'on de B y L da lugar a procesos tan indeseados como la desintegraci\'on r\'apida del prot\'on, se suele postular la existencia de una nueva simetr\'ia discreta llamada Paridad R y definida como \cite{Fayet:1974pd,Farrar:1978xj}

\begin{equation}
R_p = (-1)^{3(B-L)+2s}
\end{equation}

donde $s$ es el esp\'in de la part\'icula. Es f\'acil comprobar que esta simetr\'ia prohibe todos los t\'erminos en la ecuaci\'on \eqref{rpv-superpotential-intro}, lo que protege al prot\'on y hace desaparecer las interacciones peligrosas. Adem\'as,
el factor $(-1)^{2s}$ hace que las part\'iculas del Modelo Est\'andar y sus correspondientes compa\~neras supersim\'etricas tengan carga diferente bajo Paridad R. De hecho, puede comprobarse que todas las part\'iculas del Modelo Est\'andar tienen $R_p = +1$, mientras que sus supercompa\~neras tienen $R_p = -1$.

La consecuencia m\'as inmediata de este hecho es que, gracias a la Paridad R, la part\'icula supersim\'etrica m\'as ligera (Lightest Supersymmetric Particle, LSP) es estable, por lo que ser\'ia un buen candidato a la materia oscura del universo\footnote{De hecho, es com\'un afirmar que una de las motivaciones m\'as importantes para supersimetr\'ia es que proporciona un candidato a materia oscura. No obstante, esto no es estrictamente cierto, pues supersimetr\'ia por s\'i sola no es capaz de ello. Es la imposici\'on adicional de la Paridad R la que realiza esta funci\'on.}. Por otro lado, tambi\'en hay importantes repercusiones en f\'isica de colisionador. La conservaci\'on de Paridad R hace que las superpart\'iculas se produzcan siempre a pares y que la LSP, producida al final de todas las cadenas de desintegraci\'on, escape de los detectores sin decaer, lo que da lugar a energ\'ia perdida\footnote{La gran mayor\'ia de los estudios y simulaciones de modelos supersim\'etricos para el LHC se realizan asumiendo Paridad R conservada y, por lo tanto, la energ\'ia perdida es un elemento fundamental en los an\'alisis. Sin embargo, si Paridad R se viola y la LSP decae esta se\~nal disminuye notablemente.}.

No obstante, cabe mencionar que la inclusi\'on de esta nueva
simetr\'ia puede verse como un paso atr\'as respecto del Modelo
Est\'andar. As\'i como en aquel caso la conservaci\'on de B y L es
autom\'atica, en el MSSM se necesita a\~nadir una nueva simetr\'ia
\emph{a mano}, sin dar una motivaci\'on te\'orica que lo
justifique\footnote{Es importante se\~nalar, no obstante, que la
  conservaci\'on de B y L en el Modelo Est\'andar es puramente
  accidental. De hecho, una vez se extiende m\'inimamente para incluir
  masas no nulas para los neutrinos, la rotura de L resulta
  inmediata. Esto sucede por ejemplo cuando el espectro se extiende
  mediante la adici\'on de neutrinos dextr\'ogiros, cuyas masas de
  Majorana rompen L en dos unidades.}.

En la presente tesis se discuten dos posibles papeles de la Paridad R. Por un lado, si \'esta se rompe mediante la introducci\'on de t\'erminos que violan n\'umero lept\'onico se genera masa para los neutrinos. Esta sencilla modificaci\'on del MSSM es suficiente por lo tanto para resolver uno de los problemas abiertos del Modelo Est\'andar. En esta tesis se ha estudiado qu\'e consecuencias tiene esta idea y de qu\'e modo podemos someterla al examen experimental. Por otro lado, tambi\'en se ha estudiado la posibilidad opuesta, investigando un modelo extendido con simetr\'ia left-right que da lugar de forma autom\'atica a Paridad R a bajas energ\'ias. En ese caso la masa de los neutrinos se genera de otro modo, a trav\'es del llamado Mecanismo Seesaw, con repercusiones muy diferentes para la fenomenolog\'ia.

\section{Aspectos generales sobre modelos de masa de neutrinos}

Pasemos ahora a describir qu\'e modelos han sido propuestos para explicar el origen de la masa de los neutrinos. Antes de describir en m\'as detalle los estudiados en el desarrollo de esta tesis, discutamos brevemente algunas generalidades a tener en cuenta.

A grandes rasgos podemos clasificar los modelos de masa de neutrinos en modelos con masas de Dirac y modelos con masas de Majorana.

El primero de estos tipos puede obtenerse con una modificaci\'on realmente sencilla. Siguiendo el mismo procedimiento que se utiliza para el resto de fermiones del Modelo Est\'andar, podemos a\~nadir tres familias de neutrinos de quiralidad derecha, singletes bajo el grupo de gauge, y escribir los correspondientes acoplamientos de Yukawa

\begin{equation} \label{yuk-intro}
- \mathcal{L}_Y = Y_\nu H L \nu_R + h.c.
\end{equation}

Tras la rotura espont\'anea de la simetr\'ia electrod\'ebil este t\'ermino da lugar a masas de Dirac para los neutrinos, $m_D = Y_\nu \langle H \rangle$, al igual que los t\'erminos an\'alogos dotan de masa al resto de fermiones. En la ecuaci\'on \eqref{yuk-intro} $Y_\nu$ es una matriz $3 \times 3$. Puesto que $\langle H \rangle \sim 100$ GeV y dado que la escala absoluta para la masa de los neutrinos\footnote{La escala absoluta de la masa de los neutrinos est\'a acotada por encima gracias a observaciones cosmol\'ogicas y experimentos basados en la desintegraci\'on beta del tritio o la b\'usqueda de desintegraciones beta doble sin neutrinos. En todos los casos se obtienen cotas inferiores al eV \cite{Giunti:2005qd}.} no puede ser mayor de $1$ eV, los elementos de $Y_\nu$ deben ser inferiores a $10^{-11}$.

\begin{figure}
\begin{center}
\vspace{5mm}
\includegraphics[width=0.65\textwidth]{img/plotmasses.ps}
\end{center}
\vspace{0mm}
\caption{Masas de las part\'iculas fundamentales conocidas. Para el neutrino se utiliza el l\'imite conservador $m_\nu = 1$ eV y solamente se representa una generaci\'on. Los leptones se dibujan en azul, los quarks en rojo y los bosones de gauge masivos en verde. Los bosones de gauge sin masa, el fot\'on y el glu\'on, no est\'an incluidos en el gr\'afico.}
\label{fig:particlemasses-intro}
\end{figure}

Un valor tan peque\~no contrasta fuertemente con los Yukawas del resto de fermiones. La figura \ref{fig:particlemasses-intro} representa las masas de las part\'iculas conocidas. Para el neutrino se usa el l\'imite conservador $m_\nu = 1$ eV. Vemos que incluso en escala logar\'itmica el neutrino se encuentra muy lejos del resto de part\'iculas conocidas. Una diferencia as\'i cuesta de explicar si asumimos que el origen de las masas de estas part\'iculas es el mismo. Todo parece indicar que los neutrinos adquieren su masa de una forma diferente.

Por ello, y puesto que con acoplamientos tan peque\~nos el neutrino dextr\'ogiro ser\'ia totalmente indetectable, dar masas de Dirac a los neutrinos es una opci\'on poco popular. Por el contrario, la gran mayor\'ia de los modelos asumen que los neutrinos son part\'iculas de Majorana, es decir, sus propias antipart\'iculas.

Weinberg se\~nal\'o hace mucho tiempo que el operador no renormalizable \cite{Weinberg:1979sa}

\begin{equation} \label{wop-intro}
W_{op} = \frac{1}{\Lambda} L_i L_j H H
\end{equation}

da lugar a masas de Majorana para los neutrinos tras la rotura de la simetr\'ia electrod\'ebil. Efectivamente, cuando $\langle \phi^0 \rangle = \frac{v}{\sqrt{2}}$ se obtienen masas $m_\nu \propto \frac{v^2}{\Lambda}$, con una dependencia cuadr\'atica en el VEV $v$. En estas expresiones $\Lambda$ es la escala de energ\'ias a la que se genera el operador de Weinberg y, por lo tanto, puede ser una escala de energ\'ias muy alta. Eso explicar\'ia la peque\~nez de la masa de los neutrinos, que se ver\'ia suprimida por $\Lambda$.

Debe notarse adem\'as que el operador de Weinberg viola el n\'umero lept\'onico en dos unidades, $\Delta L = 2$. Esta es una caracter\'istica fundamental de los t\'erminos de masa de Majorana, y veremos como se repite en cada uno de los modelos estudiados.

Esta observaci\'on de Weinberg, que puede parecer trivial a simple vista, es de una gran profundidad te\'orica. De hecho, la literatura cient\'ifica est\'a llena de modelos cuyo l\'imite a bajas energ\'ias da lugar al operador de Weinberg. En concreto, existen tres realizaciones a nivel \'arbol y tres realizaciones a un loop \cite{Ma:1998dn}. De entre todas ellas la m\'as popular es el Mecanismo Seesaw en su variante Tipo-I \cite{Minkowski:1977sc,Gell-Mann:1980vs,Yanagida:1979,Mohapatra:1979ia}, la cual ha dominado completamente la literatura cient\'ifica en los \'ultimos a\~nos. En este caso se a\~naden al espectro tres familias de neutrinos dextr\'ogiros. Como ya discutimos, esto da lugar a nuevos acoplamientos de Yukawa. Sin embargo, si uno permite la introducci\'on de t\'erminos que no conservan el n\'umero lept\'onico, tambi\'en es posible escribir una masa de Majorana para \'estos, dado que son singletes bajo el grupo de gauge. Por lo tanto, los neutrinos dextr\'ogiros aparecen en los siguientes t\'erminos del lagrangiano

\begin{equation} \label{nu-lag-intro}
- \mathcal{L}_{\nu_R} = Y_\nu \phi^0 \bar{\nu}_R \nu_L + \frac{1}{2} \nu_R^T M_R \nu_R + h.c.
\end{equation}

La matriz $3 \times 3$ $M_R$ est\'a, como hemos dicho, permitida por la simetr\'ia gauge, por lo que la magnitud de sus elementos no est\'a restringida en modo alguno. Tras la rotura de la simetr\'ia electrod\'ebil se genera la masa de Dirac que mezcla a los neutrinos de quiralidad izquierda con los de quiralidad derecha, obteni\'endose la siguiente matriz de masa para los fermiones neutros

\begin{equation} \label{seesaw-matrix-intro}
M = \left( \begin{array}{c c}
0 & m_D \\
m_D^T & M_R \end{array} \right)
\end{equation}

Si asumimos $M_R \gg m_D$, esta matriz puede diagonalizarse por bloques en buena aproximaci\'on para dar lugar a tres autoestados de masa ligeros y tres pesados. De hecho, se obtiene

\begin{eqnarray}
m_{light} &=& -m_D^T \cdot M_R^{-1} \cdot m_D \\
M_{heavy} &=& M_R
\end{eqnarray}

\begin{figure}
\begin{center}
\vspace{5mm}
\includegraphics[width=0.5\textwidth]{img/seesaw-picture.eps}
\end{center}
\caption{El mecanismo seesaw explica la peque\~nez de la masa de los neutrinos mediante la introducci\'on de part\'iculas muy pesadas en la teor\'ia. De hecho, cuanto m\'as pesadas son las nuevas part\'iculas m\'as ligeros resultan los neutrinos.}
\label{fig:seesaw-picture}
\end{figure}

Por lo tanto, si la masa de Majorana de los neutrinos dextr\'ogiros es muy grande, la masa de los neutrinos ligeros es de forma natural muy peque\~na. Esta es la idea esencial tras el mecanismo seesaw\footnote{Hay otras variantes, conocidas como Tipo-II \cite{Schechter:1980gr,Konetschny:1977bn,Cheng:1980qt,Mohapatra:1980yp,Lazarides:1980nt} y Tipo-III \cite{Foot:1988aq}, en las que las part\'iculas pesadas que explican la ligereza de los neutrinos activos son otras. No obstante, la idea fundamental sigue siendo la misma.}.

Adem\'as, el mecanismo seesaw predice que los estados ligeros son, en muy buena aproximaci\'on, puramente lev\'ogiros, mientras que los pesados son dextr\'ogiros. Esto explica por qu\'e los experimentos realizados hasta la fecha han observado siempre neutrinos con quiralidad izquierda.

Por supuesto, todo lo discutido en esta secci\'on puede aplicarse tanto a modelos sin supersimetr\'ia como a modelos con ella. En ambos casos puede presentarse el mismo problema pr\'actico. Puesto que el propio seesaw requiere que los neutrinos dextr\'ogiros tengan una masa por encima de la escala electrod\'ebil, si estos son muy pesados no hay modo alguno de producirlos en un colisionador para estudiar sus propiedades. No obstante, \'este no ser\'ia el caso si, por el contrario, los neutrinos dextr\'ogiros cuentan con masas en torno al TeV. En cualquier caso, como veremos m\'as adelante, el mecanismo seesaw cuenta con ciertas ventajas una vez se a\~nade supersimetr\'ia a la teor\'ia. Esto se debe a que las superpart\'iculas, en concreto los sleptones, son sensibles a la existencia de la escala alta, obteniendo ciertas correcciones a sus masas soft que guardan memoria del seesaw \cite{Borzumati:1986qx}. Esto da lugar a procesos con violaci\'on del sabor lept\'onico, claras se\~nales de nueva f\'isica.\\

En los siguientes apartados presentamos un breve resumen de las ideas desarrolladas durante esta tesis, que caracteriza la generaci\'on de la masa de los neutrinos en varios modelos supersim\'etricos y estudia en detalle su fenomenolog\'ia en experimentos presentes y futuros.

\section{Violaci\'on de Paridad R}

El MSSM conserva Paridad R por definici\'on. Sin embargo, no hay una raz\'on te\'orica de peso que justifique esta simetr\'ia. De hecho, varios argumentos pueden usarse en contra de la imposici\'on ad-hoc de la Paridad R, v\'ease el cap\'itulo \ref{chap:rpv-intro}. Adem\'as, la violaci\'on de Paridad R es una forma muy sencilla de generar masas de neutrinos. Por ejemplo, consid\'erese el siguiente t\'ermino en el superpotencial \cite{Hall:1983id}

\begin{equation}\label{brpv-superpotential-intro}
W \supset \epsilon_i \widehat{L}_i \widehat{H}_u
\end{equation}

Este termino, que respeta todas las simetr\'ias (y supersimetr\'ias) de la teor\'ia salvo n\'umero lept\'onico, mezcla a los leptones con los higgsinos, dando lugar a un mecanismo seesaw a la escala electrod\'ebil\footnote{Como vemos, la violaci\'on de Paridad R en su forma bilineal da lugar a una realizaci\'on del mecanismo seesaw. Es un ejemplo m\'as de las diferentes realizaciones del operador de Weinberg, descripci\'on efectiva de la mayor\'ia de modelos de masa de Majorana para los neutrinos.}. Para verlo, consideremos la matriz de masa de los fermiones neutros, que incluye a los neutrinos y a los neutralinos del MSSM. Resulta

\begin{equation} \label{brpv-massF0-intro}
M_N=\left(
\begin{array}{cc}
{\cal M}_{\chi^0}& m^T \cr \vb{20} m & 0 \cr
\end{array}
\right)
\end{equation}

donde ${\cal M}_{\chi^0}$ es la matriz de masa de los neutralinos del MSSM, mientras que

\begin{equation}
m=\left(
\begin{array}{cccc}
-\frac 12g^{\prime }v_e & \frac 12g v_e & 0 & \epsilon_e \cr \vb{18}
-\frac 12g^{\prime }v_\mu & \frac 12g v_\mu & 0 & \epsilon_\mu  \cr
\vb{18} -\frac 12g^{\prime }v_\tau & \frac 12g v_\tau & 0 & \epsilon_\tau
\cr
\end{array}
\right)
\end{equation}

es la matriz que caracteriza la violaci\'on de Paridad R. En esta expresi\'on $v_i/\sqrt{2} = \langle \tilde{\nu}_i \rangle$ son los VEVs que los sneutrinos adquieren en este modelo.

N\'otese que la matriz \eqref{brpv-massF0-intro} tiene la misma estructura que la matriz \eqref{seesaw-matrix-intro}, que apareci\'o en la discusi\'on del mecanismo seesaw tipo-I. Por lo tanto, siguiendo el mismo procedimiento deducimos que si se cumple la jerarqu\'ia $m \ll {\cal M}_{\chi^0}$, se obtienen masas peque\~nas para los neutrinos.

La violaci\'on de Paridad R cambia totalmente la fenomenolog\'ia respecto a los modelos m\'as habituales. En particular, la LSP deja de ser estable y se desintegra, dejando trazas en los colisionadores. El estudio de estas se\~nales permite poner a prueba los modelos, que realizan predicciones muy precisas para ciertos observables.

Tambi\'en hay importantes implicaciones en cosmolog\'ia. Obviamente, se pierde el candidato est\'andar a materia oscura, la LSP. No obstante, hay disponibles otras bien motivadas posibilidades te\'oricas y es posible dar una explicaci\'on a la cantidad observada de materia oscura en el universo. Algunos ejemplos bien estudiados son el gravitino \cite{Borgani:1996ag,Takayama:2000uz,Hirsch:2005ag}, el axi\'on \cite{Kim:1986ax,Raffelt:1996wa} y su compa\~nero supersim\'etrico, el axino \cite{Chun:1999cq,Chun:2006ss}.

En la presente tesis se han estudiado dos modelos con violaci\'on de Paridad R. En ambos se ha extendido el modelo anteriormente discutido, conocido como violaci\'on bilineal de Paridad R, con el objetivo de solucionar algunos de sus problemas conceptuales. Por ejemplo, la jerarqu\'ia $m \ll {\cal M}_{\chi^0}$, necesaria para obtener masas de neutrinos en el rango correcto, requiere que los par\'ametros $\epsilon$ sean muy peque\~nos, lo que resulta inesperado para par\'ametros que conservan supersimetr\'ia. Diversas extensiones han aparecido a lo largo de los a\~nos para intentar explicar este detalle. La idea es a\~nadir un supercampo $\widehat S$, singlete bajo el grupo de gauge, cuya componente escalar adquiera un VEV generando un t\'ermino $\epsilon$ efectivo

\begin{equation}
\lambda_i S L_i H_u \: \to \: \lambda_i \langle S \rangle L_i H_u = \epsilon_i L_i H_u
\end{equation}

Si este VEV se genera a la escala electrod\'ebil se puede explicar f\'acilmente la peque\~nez de los par\'ametros $\epsilon_i$ usando un acoplamiento $\lambda_i \sim 10^{-7}-10^{-6}$.

Se conocen varias extensiones del modelo bilineal en esta direcci\'on. En algunas se introducen adem\'as otros t\'erminos que rompen Paridad R de forma expl\'icita, mientras que en otras la violaci\'on es espont\'anea. Las predicciones resultantes dependen en gran medida del tipo de extensi\'on realizada, aunque tambi\'en es posible encontrar algunas caracter\'isticas comunes.

En particular, todos los modelos bilineales\footnote{Llamaremos modelos bilineales a aquellos que generan la masa de los neutrinos mediante un operador del tipo $\epsilon L H_u$, tanto si \'este est\'a expl\'icitamente en el superpotencial como si se genera tras la rotura de la simetr\'ia electrod\'ebil.} cuentan con muy buenas correlaciones entre las desintegraciones de la LSP y la f\'isica de neutrinos \cite{Mukhopadhyaya:1998xj,Choi:1999tq,Romao:1999up,Porod:2000hv}. Esto no es de extra\~nar, pues la misma causa se encuentra tras los dos efectos: la rotura de Paridad R.

Si la LSP es el neutralino m\'as ligero, cocientes como $Br(\tilde{\chi}_1^0 \to W l_i)/Br(\tilde{\chi}_1^0 \to W l_j)$ son iguales a combinaciones determinadas de \'angulos de mezcla de neutrinos, por lo que es posible realizar predicciones muy precisas para experimentos de colisionador. Por ejemplo, si la LSP es predominantemente un Bino, $\tilde{\chi}_1^0 \simeq \tilde{B}^0$, obtenemos la predicci\'on

\begin{equation} \label{brpv-pred-intro}
\frac{Br(\tilde{\chi}_1^0 \to W \mu)}{Br(\tilde{\chi}_1^0 \to W \tau)} \simeq \tan^2 \theta_{23}
\end{equation}

donde $\theta_{23}$ es el \'angulo que interviene en las oscilaciones de los neutrinos atmosf\'ericos. Ahora, gracias a los ajustes globales a todos los datos experimentales disponibles \cite{Schwetz:2008er} sabemos que el \'angulo atmosf\'erico es m\'aximo, o muy cercano a ello. Por lo tanto $\tan^2 \theta_{23} \simeq 1$ y este escenario predice un n\'umero muy similar de desintegraciones al canal $\tilde{\chi}_1^0 \to W \mu$ y al canal $\tilde{\chi}_1^0 \to W \tau$. Si el neutralino tiene una composici\'on mayor en la direcci\'on de otro autoestado gauge, en algunos casos se obtiene correlaci\'on con otro \'angulo de mezcla y, por lo tanto, otra predicci\'on para los cocientes $Br(\tilde{\chi}_1^0 \to W l_i)/Br(\tilde{\chi}_1^0 \to W l_j)$. En cualquier caso, si los resultados obtenidos en un colisionador difieren de todas las posibilidades no cabr\'a duda de que el origen de la masa de los neutrinos no se encuentra en este tipo de modelos. En conclusi\'on, mediante estas se\~nales tan claras es posible poner a prueba los modelos, siendo \'este uno de los pocos casos en los que puede explorarse directamente la generaci\'on de masa de los neutrinos en un experimento.

Por otro lado, y tal y como se ha dicho, hay se\~nales que dependen claramente del modelo en cuesti\'on. A continuaci\'on describiremos brevemente los dos modelos estudiados en esta tesis y sus rasgos diferenciadores m\'as importantes.

\begin{itemize}
\item Violaci\'on espont\'anea de Paridad R
\end{itemize}

En la referencia \cite{Masiero:1990uj} se propuso un modelo cuyo lagrangiano original conserva Paridad R. No obstante, la estructura del potencial escalar es tal que ciertos campos escalares adicionales con n\'umero lept\'onico no nulo adquieren VEVs, rompiendo Paridad R a la escala electrod\'ebil y generando la masa de los neutrinos. 

Estos supercampos con n\'umero lept\'onico, llamados $\widehat \nu^c$ y $\widehat S$ en \cite{Masiero:1990uj}, son singletes bajo el grupo de gauge, lo cual resulta de gran utilidad para evitar los fuertes l\'imites experimentales que han servido para descartar modelos previos \cite{Aulakh:1982yn}. La raz\'on est\'a en que al romper Paridad R se rompe tambi\'en la simetr\'ia global $U(1)_L$, el n\'umero lept\'onico, por lo que aparece un bos\'on de Goldstone en el espectro. Si este bos\'on de Goldstone, llamado major\'on ($J$) \cite{Chikashige:1980ui,Gelmini:1980re}, tuviera carga bajo el grupo de gauge, contribuir\'ia a numerosos procesos fuertemente acotados, lo que descarta dichos modelos. Por el contrario, romper el n\'umero lept\'onico con singletes es una opci\'on totalmente compatible con la fenomenolog\'ia.

El major\'on provoca numerosas se\~nales novedosas. Adem\'as de contar con las desintegraciones de la LSP correlacionadas con la f\'isica de neutrinos, la posibilidad de producir majorones en el colisionador y su consiguiente fuga sin ser detectados (dadas sus d\'ebiles interacciones con la materia) da lugar a desintegraciones invisibles. Por ejemplo, un neutralino LSP puede decaer seg\'un $\tilde{\chi}_1^0 \to J \nu$, escapando tanto el major\'on como el neutrino del detector sin dejar huella. Esto puede hacer que se confunda el modelo con el MSSM con Paridad R conservada, ya que al no dejar rastro de su desintegraci\'on, se simula una LSP estable\footnote{En las referencias \cite{Hirsch:2004rw,Hirsch:2005wd} se discute tambi\'en la posibilidad de que el bos\'on de Higgs se desintegre de forma invisible seg\'un $h^0 \to J J$, encontrando importantes regiones del espacio de par\'ametros en las que este canal resulta dominante. Por supuesto, esto trastocar\'ia totalmente todas las estrategias de b\'usqueda en el LHC.}.

De hecho, tal y como se investig\'o en la referencia \cite{Hirsch:2008ur}, hay regiones del espacio de par\'ametros en que esta desintegraci\'on es dominante. Cuanto m\'as baja sea la escala de rotura del n\'umero lept\'onico, m\'as alto es el cociente de desintegraci\'on a este canal, que puede alcanzar valores superiores al 99\%. Por ello, en dichas regiones del espacio de par\'ametros ser\'a necesaria (i) una muy buena estad\'istica que pueda discriminar los pocos eventos con desintegraciones visibles, y/o (ii) se\~nales adicionales que permitan distinguir del MSSM.

En esta tesis se ha abordado el problema tomando la segunda estrategia, mostrando que la desintegraci\'on de los muones puede ser sensible a la existencia de majorones. Procesos como $\mu \to e J$ o $\mu \to e J \gamma$ son m\'as probables si la escala de rotura de la Paridad R es baja, justamente la regi\'on del espacio de par\'ametros donde m\'as dificultades hay para distinguir el modelo del MSSM \cite{Hirsch:2009ee}. En concreto, se ha estudiado el posible uso del experimento MEG \cite{meg} para acotar estas desintegraciones ex\'oticas del mu\'on y c\'omo, en combinaci\'on con las se\~nales de colisionador, se puede diferenciar el modelo.

\begin{itemize}
\item $\mu\nu$SSM
\end{itemize}

Por su parte, el $\mu\nu$SSM fue propuesto recientemente en \cite{LopezFogliani:2005yw} como un modelo de masa de neutrinos muy econ\'omico. La idea fundamental es emplear el neutrino dextr\'ogiro como singlete del NMSSM, escribiendo un superpotencial que incluya los t\'erminos

\begin{equation}
{\cal W} \supset Y_{\nu} \widehat L \widehat \nu^c \widehat H_u - \lambda \widehat \nu^c \widehat H_d \widehat H_u +\frac{\kappa}{3!} (\widehat{\nu}^c)^3
\end{equation}

De este modo, al tiempo que se tiene el Yukawa de los neutrinos habitual, tambi\'en se introduce el t\'ermino $\lambda \widehat \nu^c \widehat H_d \widehat H_u$. Tras romperse la simetr\'ia electrod\'ebil y generarse el VEV $\langle \tilde{\nu}^c \rangle$, estos dos t\'erminos dan lugar al t\'ermino $\epsilon$ del modelo bilineal y al t\'ermino $\mu$ del MSSM, respectivamente. Si introducimos los \'indices de familia, \'estos resultan

\begin{eqnarray}
\epsilon_i &=& Y_\nu^{ij} \frac{v_{Rj}}{\sqrt{2}} \\
\mu &=& \lambda_i \frac{v_{Ri}}{\sqrt{2}}
\end{eqnarray}

donde $\langle \tilde{\nu}_i^c \rangle = \frac{v_{Ri}}{\sqrt{2}}$. Si $v_{Ri} \sim 100$ GeV entonces con $Y_\nu^{ij} \sim 10^{-7}-10^{-6}$ y $\lambda_i \sim 1$ se obtienen los par\'ametros en el rango deseado.

N\'otese que la presencia simult\'anea de estos operadores hace que la violaci\'on de Paridad R sea ahora expl\'icita y por lo tanto no aparece un major\'on. No obstante, la fenomenolog\'ia contiene numerosas se\~nales no est\'andar. En cierto modo, puede decirse que la fenomenolog\'ia del $\mu\nu$SSM combina violaci\'on de Paridad R, con desintegraciones de la LSP y correlaciones con los \'angulos de mezcla de los neutrinos, y del NMSSM, con la posibilidad de tener singletes ligeros y cambios dr\'asticos respectos del MSSM. En la referencia \cite{Bartl:2009an}, parte importante de esta tesis, se estudiaron en detalle las se\~nales que el $\mu\nu$SSM tiene en experimentos de colisionador, mostrando cu\'ales son m\'as relevantes en cada parte del espacio de par\'ametros.

En cualquier caso, sea la rotura del n\'umero lept\'onico espont\'anea o expl\'icita, los modelos con violaci\'on de Paridad R ofrecen una rica fenomenolog\'ia, con numerosas se\~nales visibles y claras desviaciones respecto de los modelos que conservan Paridad R. Adem\'as, son una extensi\'on del MSSM muy sencilla, y aun as\'i pueden explicar de forma sencilla la masa de los neutrinos. Por todo ello, no cabe duda sobre su justificaci\'on.

\section{Modelos Left-Right y violaci\'on del sabor lept\'onico a bajas energ\'ias}

La segunda parte de la tesis aborda la generaci\'on de masa de los neutrinos desde un punto de vista bien diferente. Si Paridad R es una simetr\'ia conservada uno debe dar respuesta a dos cuestiones fundamentales:  (1) cu\'al es el modo en que se genera la masa de los neutrinos, y (2) cu\'al es el origen de Paridad R.

Como ya se ha comentado, el mecanismo seesaw es una opci\'on muy popular para generar las masas de los neutrinos. Al considerar neutrinos dextr\'ogiros muy pesados se explica la peque\~nez de la masa de los neutrinos activos, observados en nuestros experimentos, al tiempo que se conecta con escalas de energ\'ias muy altas, cercanas a la hipot\'etica escala de gran unificaci\'on.

De hecho, el mecanismo seesaw cuenta con importantes motivaciones te\'oricas, tales como su presencia en modelos basados en simetr\'ias left-right o $SO(10)$. El hecho de que los neutrinos dextr\'ogiros, singletes bajo el grupo de gauge del Modelo Est\'andar, sean muy pesados parece una opci\'on razonable si su masa procede de una teor\'ia con un grupo de simetr\'ia m\'as amplio. 

Sin embargo resulta muy dif\'icil, si no imposible, someter el mecanismo seesaw al juicio experimental. La raz\'on est\'a en el propio coraz\'on de la idea. La existencia de part\'iculas muy masivas es una posibilidad muy natural para explicar la masa de los neutrinos, pero al mismo tiempo impide que los aceleradores de part\'iculas actuales, o incluso futuros, puedan fabricarlas para su posterior estudio.

No obstante, ciertos trabajos recientes \cite{Buckley:2006nv,Hirsch:2008dy,Hirsch:2008gh,Esteves:2009vg} han se\~nalado que en determinados escenarios supersim\'etricos es posible obtener se\~nales indirectas que conecten el mecanismo de seesaw con observables de colisionador a la escala electrod\'ebil. Ejemplos de ello son relaciones entre masas de superpart\'iculas o cocientes de desintegraci\'on de sleptones, cantidades medibles en el LHC u otros colisionadores, que pueden abrir una ventana hacia la alta escala de energ\'ias a la que se da el mecanismo seesaw.

Dicha conexi\'on se debe a las ecuaciones del grupo de renormalizaci\'on (Renormalization Group Equations, RGE) de la teor\'ia. Cuando la teor\'ia subyacente es supersim\'etrica y contiene el mecanismo de seesaw las RGE provocan que la mezcla en el sector de neutrinos se traduzca en la existencia de par\'ametros soft con violaci\'on de sabor lept\'onico en el sector de sleptones \cite{Borzumati:1986qx}. Este efecto tiene consecuencias observables en experimentos presentes como MEG\footnote{Esta conexi\'on entre la generaci\'on de masa de los neutrinos y la violaci\'on de sabor en los par\'ametros soft puede verse oscurecida si dichos par\'ametros no obedecen una condici\'on de universalidad a una cierta escala alta. No obstante, la hip\'otesis de universalidad se encuentra muy bien motivada desde el punto de vista te\'orico, tal y como veremos m\'as adelante.}.

En la presente tesis se ha seguido la idea anterior estudiando su aplicaci\'on en modelos seesaw no m\'inimos, ligando la generaci\'on de masa de los neutrinos con la obtenci\'on de Paridad R a bajas energ\'ias. Para ello se ha investigado el origen de Paridad R y su conexi\'on con teor\'ias supersim\'etricas left-right \cite{Mohapatra:1974gc,Senjanovic:1975rk,Cvetic:1983su}. Estas teor\'ias cuentan con una motivaci\'on m\'as all\'a de Paridad R. De hecho, fueron inventadas a finales de los 70 como una extensi\'on del Modelo Est\'andar que restaura la simetr\'ia Paridad a altas energ\'ias. El grupo de gauge se extiende a $SU(3)_c \times SU(2)_L \times SU(2)_R \times U(1)_{B-L}$ y por lo tanto se conserva Paridad R autom\'aticamente en el r\'egimen en que la teor\'ia es exacta, debido a la inclusi\'on de la pieza $U(1)_{B-L}$.

Puesto que la conservaci\'on de Paridad R en los modelos m\'inimos es un asunto controvertido, v\'eanse las referencias \cite{Kuchimanchi:1993jg,Babu:2008ep}, el trabajo desarrollado en esta tesis se ha llevado a cabo en un modelo no m\'inimo \cite{Aulakh:1997ba,Aulakh:1997fq} que incluye dos supercampos adicionales $\widehat{\Omega}$ y $\widehat{\Omega}^c$, donde $\widehat{\Omega}(1,3,1,0)$ y $\widehat{\Omega}^c(1,1,3,0)$ bajo $SU(3)_c \times SU(2)_L \times SU(2)_R \times U(1)_{B-L}$. La introducci\'on de estos nuevos grados de libertad hace que el potencial escalar disponga de m\'as libertad, lo que ha hecho posible demostrar la existencia de m\'inimos que conservan Paridad R.

Es importante resaltar que los modelos con simetr\'ia left-right incorporan autom\'aticamente neutrinos dextr\'ogiros. Esto se debe precisamente a la restauraci\'on de la simetr\'ia paridad, que requiere introducir representaciones del subgrupo $SU(2)_R$ an\'alogas a las que se introducen para el subgrupo $SU(2)_L$. En el caso de los leptones esto implica que adem\'as de los dobletes de $SU(2)_L$ habituales

\begin{equation}
L = \left( \begin{array}{c}
\nu \\
e \end{array} \right)
\end{equation}

uno cuenta con dobletes de $SU(2)_R$

\begin{equation}
L^c = \left( \begin{array}{c}
e^c \\
- \nu^c \end{array} \right)
\end{equation}

que incluyen al neutrino dextr\'ogiro $\nu^c$. Por lo tanto, la variante tipo-I del mecanismo seesaw puede ser implementada naturalmente en estos modelos\footnote{Hay un detalle adicional a tener en cuenta. Puesto que la pieza $U(1)_{B-L}$ tambi\'en forma parte del grupo left-right, la masa de Majorana de los neutrinos dextr\'ogiros est\'a prohibida por invariancia gauge. Sin embargo, \'esta puede generarse si se rompe la simetr\'ia $U(1)_{B-L}$ de forma apropiada, con VEVs de campos que tengan carga $B-L = 2$. \'Este es el caso considerado en esta tesis.}.

El resultado de este trabajo ha mostrado que, adem\'as de las predicciones habituales en modelos seesaw supersim\'etricos, se obtienen algunas se\~nales caracter\'isticas que distinguen al modelo en cuesti\'on. En particular, y dado que el modelo estudiado tiene una simetr\'ia left-right, se ha investigado la novedosa posibilidad de obtener violaci\'on de sabor lept\'onico en el sector right, algo que jam\'as se da en los modelos seesaw m\'inimos. De este modo, al mismo tiempo que se enlaza la masa de los neutrinos con la f\'isica de colisionador, se obtiene informaci\'on muy relevante sobre la estructura de la teor\'ia a escalas muy altas.

De hecho, esta observaci\'on es bastante sencilla. La simetr\'ia left-right se encarga de hacer que las masas soft de los sleptones left, $m_L^2$, y los sleptones right, $m_{L^c}^2$, obtengan contribuciones iguales desde la escala de gran unificaci\'on, $m_{GUT}$, hasta la escala $v_R$ a la que se rompe paridad. Un c\'alculo aproximado al orden dominante da como resultado

\begin{eqnarray}
\Delta m_L^2 &=& - \frac{1}{4 \pi^2} \left( 3 f f^\dagger + Y_L^{(k)} Y_L^{(k) 
\: \dagger} \right) (3 m_0^2 + A_0^2) \ln \left( \frac{m_{GUT}}{v_R} \right) \label{rg1-intro} \\
\Delta m_{L^c}^2 &=& - \frac{1}{4 \pi^2} \left( 3 f^\dagger f + Y_L^{(k) 
\: \dagger} Y_L^{(k)} \right) (3 m_0^2 + A_0^2) \ln \left( \frac{m_{GUT}}{v_R} \right) \label{rg2-intro}
\end{eqnarray}

En estas expresiones $Y_L^{(k)}$ son los correspondientes acoplamientos de Yukawa que describen la interacci\'on con los bidobletes de Higgs a energ\'ias superiores a $v_R$. El resto de par\'ametros se definen en detalle en el cap\'itulo \ref{chap:susylr}.

A la vista de las ecuaciones \eqref{rg1-intro} y \eqref{rg2-intro}, resulta evidente que, al igual que se encuentran efectos de violaci\'on de sabor lept\'onico en el sector left, del mismo modo debe ser posible en el sector right.

Observables interesantes en este sentido son las desintegraciones de sleptones con violaci\'on de sabor, tales como $\tilde{\tau}_i \to \tilde{\chi}_1^0 \mu$. A diferencia del seesaw m\'inimo, esta tesis demuestra que los sleptones right pueden contar tambi\'en con cocientes de desintegraci\'on medibles a canales que violan el sabor lept\'onico, lo que supone una interesante distinci\'on. Del mismo modo, la diferencia entre las masas de los sleptones de las primeras dos generaciones es tambi\'en muy sensible a nuestras modificaciones, obteni\'endose de nuevo diferencias medibles en el sector right en contraste con el caso habitual.

Finalmente, tambi\'en se ha encontrado una clara desviaci\'on respecto al seesaw m\'inimo en otro observable. Se trata de la polarizaci\'on de los positrones en la desintegraci\'on $\mu^+ \to e^+ \gamma$, proceso que est\'a siendo buscado por el experimento MEG. Efectivamente, midiendo la distribuci\'on angular de los positrones producidos es posible distinguir entre positrones con polarizaci\'on izquierda y positrones con polarizaci\'on derecha, pudi\'endose medir la asimetr\'ia $\mathcal{A}(\mu^+ \to e^+ \gamma)$, definida como

\begin{equation}
\mathcal{A}(\mu^+ \to e^+ \gamma) = \frac{|A_L|^2-|A_R|^2}{|A_L|^2+|A_R|^2}
\end{equation}

Aqu\'i $A_L$ y $A_R$ son los acoplamientos generados por los sleptones left y right, respectivamente. En el seesaw m\'inimo se espera $\mathcal{A} = +1$ en muy buena aproximaci\'on, dado que la violaci\'on de sabor solamente aparece en el sector left. En nuestro estudio, por el contrario, se muestra que desviaciones respecto a esta predicci\'on son posibles debido a la nueva violaci\'on de sabor en el sector right, y por lo tanto $\mathcal{A} < 1$ ser\'ia un claro indicio de una simetr\'ia left-right a escalas altas de energ\'ia.

\section{Conclusiones}

El objeto de esta tesis es la fenomenolog\'ia de modelos de masa de neutrinos en supersimetr\'ia. Se han empleado tanto herramientas anal\'iticas como num\'ericas en la investigaci\'on en que se basa esta tesis, cuyos resultados han sido descritos en los cap\'itulos previos. En las l\'ineas a continuaci\'on se sumarizan las principales conclusiones y se presenta una imagen global de la tesis.

Dos alternativas diferentes para generar masas de los neutrinos han sido estudiadas en esta tesis: (1) modelos con violaci\'on de Paridad R y rotura de n\'umero lept\'onico, y (2) modelos supersim\'etricos left-right que conservan Paridad R a bajas energ\'ias. En ambos casos se ha realizado un estudio detallado de la fenomenolog\'ia, obteniendo predicciones num\'ericas para experimentos presentes y futuros.

Se ha puesto m\'as \'enfasis en la falsabilidad de los modelos que en su verificaci\'on. De hecho, es imposible verificar un modelo. En este sentido, la idea de ciencia de Popper ha sido aplicada a lo largo de esta tesis, buscando se\~nales experimentales claras que, de no ser observadas, descarten los modelos investigados.

En la primera parte de la tesis se ha investigado la fenomenolog\'ia de dos modelos con violaci\'on de Paridad R. En este marco los neutrinos obtienen masas debido a su mezcla con los higgsinos en lo que puede considerarse una versi\'on electrod\'ebil del mecanismo seesaw. La m\'as limpia de las predicciones en este tipo de modelos es la pronunciada correlaci\'on que se encuentra entre las desintegraciones de la LSP y la f\'isica de neutrinos. Esto puede usarse para descartar el modelo en colisionadores si se encontrara una desviaci\'on clara respecto de los cocientes predichos.

Cuando la Paridad R se rompe espont\'aneamente un bos\'on de Goldstone aparece en el espectro, el llamado major\'on. Esto conduce a muchas se\~nales novedosas, algunas de las cuales han sido estudiadas en esta tesis. Encontramos que las desintegraciones invisibles de la LSP pueden ser dominantes si la escala de rotura del n\'umero lept\'onico es baja. Esto requerir\'ia una gran estad\'istica para distinguir s-\rpv del MSSM con Paridad R conservada. Sin embargo, si los experimentos de bajas energ\'ias son tenidos en cuenta nuevas perspectivas aparecen. La b\'usqueda de desintegraciones ex\'oticas del mu\'on involucrando majorones en el estado final es de gran ayuda para resolver la confusi\'on potencial, pues los cocientes de desintegraci\'on para estos procesos se incrementan en la misma regi\'on del espacio de par\'ametros donde la LSP se desintegra principalmente a canales invisibles.

Si, por otro lado, la Paridad R se rompe de forma expl\'icita, no se genera major\'on alguno en el modelo. Este es el caso del $\mu\nu$SSM el cual, no obstante, tiene una muy rica fenomenolog\'ia en colisionadores. Combina las claras correlaciones encontradas en los modelos con violaci\'on bilineal de Paridad R con la interesante posibilidad, tambi\'en presente en el NMSSM, de un singlete ligero. En esta tesis se describe la fenomenolog\'ia del $\mu\nu$SSM con una o dos generaciones de supercampos singletes, junto con la caracterizaci\'on de las masas de los neutrinos en ambos casos.

La segunda parte de esta tesis est\'a dedicada al estudio de un modelo supersim\'etrico left-right no m\'inimo que conduce a la conservaci\'on de Paridad R a bajas energ\'ias. En este caso las masas de los neutrinos se generan con un mecanismo seesaw tipo-I.

El modelo se describe en detalle y sus RGEs se calculan a nivel de 2-loops incluyendo correciones de umbral a las escalas intermedias. Esto se implemente num\'ericamente con la ayuda de herramientas como Sarah y SPheno, las cuales han sido usadas extensivamente en esta tesis. El c\'odigo resultante es capaz de calcular las masas soft de los sleptones a la escala SUSY y, como es habitual, la inclusi\'on del mecanismo seesaw provoca la aparici\'on de entrantes no diagonales en estas matrices. Como consecuencia de ello, se obtienen se\~nales con violaci\'on de sabor lept\'onico a la escala SUSY.

Sin embargo, adem\'as de la fenomenolog\'ia conocida en el sector de los sleptones left, hemos encontrado se\~nales en el de los right, lo que claramente indica una implementaci\'on del seesaw no m\'inima. Observables como las desintegraciones con violaci\'on de sabor lept\'onico de los sleptones, sus diferencias de masas o la asimetr\'ia en la polarizaci\'on del positr\'on en $\mu^+ \to e^+ \gamma$ diferente de $\mathcal{A}=+1$, ser\'ian claros indicios de una simetr\'ia left-right subyaciente.

Adem\'as, medidas de cocientes como $Br(\tilde{\tau}_R \to \tilde{\chi}_1^0 \mu)/Br(\tilde{\tau}_L \to \tilde{\chi}_1^0 \mu)$ limitan la estructura del modelo a altas energ\'ias, puesto que est\'an correlacionados con el cociente $v_{BL}/v_R$. No obstante, un conocimiento preciso del espectro es necesario si uno quiere poner fuertes y fiables cotas.

Finalmente, otros observables cambian ligeramente con respecto a los modelos seesaw m\'inimos. \'Este es el caso de $\mu \to e \gamma$, cuyo cociente de desintegraci\'on se incrementa debido a las nuevas contribuciones procedentes de los sleptones right.

Como conclusi\'on general de esta tesis, las masas de los neutrinos nos hacen pensar que se encontrar\'a una rica fenomenolog\'ia en el LHC y otros experimentos en marcha. Solamente mediante el examen cuidadoso de los nuevos datos podremos desenredar las diferentes se\~nales y descubrir cu\'al de nuestros modelos, si acaso alguno, es la descripci\'on correcta de la naturaleza.


==> latenumass.tex <==
In this Section we are going to introduce some definitions related with horizons of BHs, and we are going to discuss an application of the characteristic analysis to the inner boundary conditions of trapping horizons.

\section{Definitions of horizons}
The definitions and calculations of this part have been taken from \cite{GJ}, in which all the details can be found.

Let a hypersurface $\Hor$ of ${\cal M}$ be the image of a 3-dimensional manifold $\Hor_0$ by an embedding $\Phi:\Hor_0 \rightarrow \M$, $\Hor = \Phi\left(\Hor_0\right)$. The pull-back of the bilinear form \w{$g$}, i.e. the spacetime metric, defines the induced metric on $\Hor$, also called the first fundamental form of $\Hor$: \w{$q$}$:=\Phi^*$\w{$g$}. The hypersurface $\Hor$ is said to be null if, and only if, the induced metric \w{$q$} is degenerate; this means if, and only if, there exists a vector field \w{$l$} in $\T\left(\Hor\right)$, the space of smooth vector fields on $\M$, that satisfies $\forall$\w{$v$} $\in\T\left(\Hor\right)$, \w{$q$}(\w{$l$},\w{$v$})$=0$. In null hypersurfaces their normal vectors are both orthogonal and tangent to them.

For any hypersurface, the \textquotedblleft bending\textquotedblright of $\Hor$ in $\M$ or extrinsic curvature of $\Hor$ is described by the Weingarten map or shape operator, which is the endomorphism of $\T_p\left(\Hor\right)$, the tangent space of vectors at $p$, which associates to each vector tangent to $\Hor$ the variation of the normal \w{$l$} along that vector, with respect to the space-time connection \w{$\nabla$}:
\bea
	\w{\chi}:\T_p\left(\Hor\right) & \longrightarrow & \T_p\left(\Hor\right) \nonumber \\
	v & \longmapsto & \w{\nabla}_v \w{l}
\eea
This application is well defined since $\w{l}\cdot\w{\chi}\left(v\right)=\w{l}\cdot\w{\nabla}_v\w{l}= 1/2\ \w{\nabla}_v\left(\w{l}\cdot\w{l}\right)=0$. The Weingarten map depends on the specific choice of the normal \w{$l$}; a rescaling of \w{$l$} acts as follows on \w{$\chi$}: $\w{l}\rightarrow\w{l}'=\alpha\w{l}\Rightarrow\w{\chi}\rightarrow\w{\chi}'=\alpha\w{\chi}+\left\langle \w{d}\alpha,\cdot\right\rangle\w{l}$. The fundamental property of this application is to be self-adjoint with respect to the metric \w{$q$}.

This property implies the symmetry of the bilinear form defined on $\Hor$'s tangent space by:
\bea
	\w{\Theta}:\T_p\left(\Hor\right)\times\T_p\left(\Hor\right) & \longrightarrow & \mathbb{R} \nonumber \\
	\left(u,v\right) & \longmapsto & u\cdot\w{\chi}\left(v\right)
\eea
It is called the second fundamental form of $\Hor$ with respect to \w{$l$}. It is symmetric only because \w{$l$} is normal to some hypersurface. Actually, it is nothing but the pull-back of the bilinear form \w{$\nabla \underline{l}$} onto $\T_p\left(\Hor\right)$ induced by the embedding $\Phi$ of $\Hor$ in $\M$: \w{$\Theta=\Phi^*\nabla \underline{l}$}. As for \w{$\chi$}, \w{$\Theta$} depends on the choice of the normal \w{$l$}; its transformation under a rescaling of \w{$l$} is: $\w{l}\rightarrow\w{l}'=\alpha\w{l}\Rightarrow\w{\Theta}\rightarrow\w{\Theta}'=\alpha\w{\Theta}$.

If we take into account the foliation provided by the family of spacelike hypersurfaces that foliates the space-time in the 3+1 formalism, we have some extra-structure on $\M$. From now on, $\Hor$ is assumed to be a null hypersurface. We will define unambiguously a transverse direction to $\Hor$ and an associated projector \w{$\Pi$}.

Each spacelike hypersurface $\Sigma_t$ of the 3+1 slicing intersects the null hypersurface $\Hor$ on some 2-dimensional surface: $\Sp_t:=\Hor\cap\Sigma_t$. As a submanifold of $\Sigma_t$, each $\Sp_t$ is necessarily a spacelike surface. The $\Sp_t$'s constitute a foliation on $\Hor$. The coordinate $t$ can then be used as a parameter. We can normalize the null normal \w{$l$} of $\Hor$ by demanding that \w{$l$} is the tangent vector associated with this parametrization, or equivalently demanding that \w{$l$} is a vector field dual to the 1-form $\w{d}t:\w{\nabla}_{\w{l}}t=1$.

Let \w{$s$} be the unit vector of $\Sigma_t$, normal to $\Sp_t$ and directed towards the exterior of $\Sp_t$.
Let $\w{b}\in\T_p\left(\Sp_t\right)$, $\w{b}:=\vec{\w{\gamma}}\left(\w{l}\right)$. Due to the normalization on the null normal \w{$l$}, it can be expressed as $\w{l}=N\w{n}+\w{b}$. It can be deduced that \w{$b$} is a vector of $\Sigma_t$ which is normal to $\Sp_t$; then it is necessarily colinear to \w{$s$}. Because \w{$l$} is null, $\w{l}=N\left(\w{n}+\w{s}\right)$. Since $\vec{\w{\gamma}}\left(\w{l}\right)=N\w{s}$ with $N>0$, we say that \w{$l$} is an outgoing null vector with respect to $\Sp_t$.

We need some direction transverse to $\Hor$ to define a projector. The slicing has already provided the timelike direction \w{$n$} and the spacelike direction \w{$s$}, both normal to the 2-surfaces $\Sp_t$. We may also think about the null directions normal to $\Sp_t$. The ingoing direction is defined by the null vector $\w{k}= 1/2N\ \left(\w{n}-\w{s}\right)$. This null vector satisfies $\w{l}\cdot\w{k}=-1$. Each pair $\left(\w{n},\w{s}\right)$ or $\left(\w{l},\w{k}\right)$ forms a basis of the vectorial plane orthogonal to $\Sp_t$.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=10cm,height=6cm]{ericjl.eps}
\caption{Null vector $\w{l}$ normal to $\Hor$, unit timelike vector $\w{n}$ normal to $\Sigma_t$, unit spacelike vector $\w{s}$ normal to $\Sp_t$ and ingoing null vector $\w{k}$ normal to $\Sp_t$, from \cite{GJ}.}
\end{center}
\end{figure}

We can now define the projector onto $\Hor$ along \w{$k$} by:
\bea
	\w{\Pi}:\T_p\left(\M\right) & \longrightarrow & \T_p\left(\Hor\right) \nonumber \\
	v & \longmapsto & v + \left(\w{l}\cdot v\right)\w{k}
\eea
It is well defined. It leaves invariant any vector in $\T_p\left(\Hor\right)$. It satisfies $\w{\Pi}\left(\w{k}\right)=0$ and $\w{\Pi}\left(\w{l}\right)=\w{l}$. Its definition does not depend on the normalization of \w{$l$} and \w{$k$} as long as they satisfy the relation $\w{l}\cdot\w{k}=-1$; the application is determined only by the foliation $\Sp_t$ of $\Hor$ and not by the scale of $\Hor$'s null normal.

Once introduced the projector \w{$\Pi$} onto $\Hor$, we can extend the definition of the Weingarten map of $\Hor$ to all vectors of $\T_p\left(\M\right)$ by:
\bea
	\w{\chi}:\T_p\left(\M\right) & \longrightarrow & \T_p\left(\Hor\right) \nonumber \\
	v & \longmapsto & \w{\chi}_{\Hor}\left(\w{\Pi}\left(v\right)\right),
\eea
where $\w{\chi}_{\Hor}$ denotes de Weingarten map introduced on $\T_p\left(\Hor\right)$.
Similary, we make use of the projector to extend the definition of the second fundamental form of $\Hor$ with respect to the normal \w{$l$} by $\w{\Theta}:=\w{\Pi}^*\w{\Theta}_{\Hor}$, where $\w{\Theta}_{\Hor}$ denotes the second fundamental form of $\Hor$ with respect to \w{$l$} introduced before; explicitly:
\bea
	\w{\Theta}:\T_p\left(\M\right)\times\T_p\left(\M\right) & \longrightarrow & \mathbb{R} \nonumber \\
	\left(u,v\right) & \longmapsto & \w{\Theta}_{\Hor}\left(\w{\Pi}\left(u\right), \w{\Pi}\left(v\right)\right).
\eea
Actually, it is nothing but the pull-back of the bilinear form {\w$\nabla \underline{l}$} onto $\T_p\left(\M\right)$ induced by the projector $\vec{\w{q}}$: {\w$\Theta=\vec{q}^*\nabla \underline{l}$}. The bilinear form \w{$\Theta$} has at least two degeneracy directions, \w{$l$} and \w{$k$}; then, we can conclude that any vector in the plane orthogonal to $\Sp_t$ is also a degeneracy direction for \w{$\Theta$}.

We define the tensor of deformation rate with respect to \w{$l$} of the 2-surface $\Sp_t$ as half the Lie derivative of $\Sp_t$'s metric \w{$q$} along the vector field \w{$l$}: $\w{Q}:=1/2\ ^\Sp\Liec{l}\w{q}$, where \w{$q$} is considered as a bilinear form field on $\Sp_t$ and $^\Sp\Liec{l}$ is the Lie derivative intrinsic to $\Sp_t$ which arises from the Lie-dragging of $\Sp_t$ by \w{$l$}. It can be deduced that:
\be
\label{e:otradef}
	\w{\Theta} = \vec{\w{q}}^*\w{Q} = \frac{1}{2}\vec{\w{q}}^*\:^\Sp{\cal L}_{\w{l}}\w{q} = \frac{1}{2}\vec{\w{q}}^*\Liec{l}\w{q}.
\ee

Let us split the second fundamental form, now considered as the deformation rate of the 2-surfaces $\Sp_t$, into a trace part and a traceless part with respect to $\Sp_t$'s metric \w{$q$}:
\be
	\w{\Theta} = \frac{1}{2}\theta\w{q} + \w{\sigma},
\ee
where
\bea
	\theta & := & {\mathrm tr} \vec{\w{\Theta}}, \\
	\w{\sigma} & := & \w{\Theta}-\frac{1}{2}\theta\w{q},
\eea
are the trace of the endomorphism $\vec{\w{\Theta}}$ canonically associated with $\w{\Theta}$ by the metric \w{$g$} and \w{$\sigma$} is the traceless part of $\w{\Theta}$ respectively. The trace $\theta$ is called the expansion scalar of $\Sp_t$ and \w{$\sigma$} the shear tensor of $\Sp_t$. If we denote by $q$ the determinant of the components of the metric \w{$q$} with respect to the coordinates in $\Sp_t$, the expansion scalar satisfies $\theta =\:^\Sp\Liec{l}\ln\sqrt{q}$, that justifies its name, for $\sqrt{q}$ is related to the surface element $^2\epsilon$ of $\Sp_t$. $\theta$ depends only upon the null normal \w{$l$} to ${\cal H}$, so the dependence of $\theta$ with respect to the foliation $\Sp_t$ is only through the normalization of \w{$l$} induced by the $\Sp_t$ slicing and not on the precise shape of this slicing.

By analogy with the expression (\ref{e:otradef}) of \w{$\Theta$}, we define the transversal deformation rate of the 2-surface $\Sp_t$ as the projection onto $\T\left(\Sp_t\right)$ of the Lie derivative of $\Sp_t$'s metric \w{$q$} along the null transverse vector \w{$k$}:
\be
	\w{\Xi} := \frac{1}{2}\vec{\w{q}}^*\Liec{k}\w{q},
\ee
where \w{$q$} is considered as 4-dimensional bilinear form, and $\Liec{k}\w{q}$ is its Lie derivative within the 4-manifold ${\cal M}$. Since the vector field \w{$k$} does not Lie drag the surfaces $\Sp_t$, we do not have an object such as the 2-dimensional Lie derivative analog of $^\Sp\Liec{l}$. It can be deduced that $\w{\Xi}=\vec{\w{q}}^*\w{\nabla}\underline{\w{k}}$. A rescaling of \w{$l$} acts as follows: \linebreak $\w{l}\rightarrow\w{l}'=\alpha\w{l}\Rightarrow\w{\Xi}\rightarrow\w{\Xi}'=\alpha^{-1}\w{\Xi}$.

Similary to the definition of the expansion scalar $\theta$ as the trace of the deformation rate \w{$\Theta$}, we define the transversal expansion scalar $\theta_{\left(k\right)}$ as the trace of \w{$\Xi$}

We say that the null hypersurface ${\cal H}$ is a non-expanding horizon (NEH) if, and only if, the following properties hold:
\begin{enumerate}[(i)]
	\item ${\cal H}$ has the topology of $\mathbb{R}\times\mathbb{S}^2$;
	\item the expansion scalar $\theta$ vanishes on ${\cal H}$: $\theta\stackrel{\cal H}{=}0$;
	\item the matter stress-energy tensor \w{$T$} obeys the null dominant energy condition on ${\cal H}$, namely the \textquotedblleft energy-momentum current density\textquotedblright vector $\w{W}:=-\vec{\w{T}}\cdot\w{l}$ is future directed timelike or null on ${\cal H}$.
\end{enumerate}
Properties (ii) and (iii) do not depend upon the choice of a specific null normal \w{$l$}; the property of being a NEH is an intrinsic property of the null hypersurface ${\cal H}$, and in particular it does not depend upon the space-time foliation by the hypersurfaces $\Sigma_t$.

A trapped surface has been defined by Penrose (1965) as a closed (i.e. compact without boundary) spacelike 2-surface $\Sp$ such that the two systems of null geodesics emerging orthogonally from $\Sp$ converge locally at $\Sp$, i.e. they have non-positive scalar expansions. In the present context, demanding that the spacelike 2-surface $\Sp_t={\cal H}\cap\Sigma_t$ be a trapped surface is equivalent to $\theta\leq0$ and $\theta_{\left(k\right)}\leq0$. The subcase $\theta=0$ or $\theta_{\left(k\right)}=0$ is referred to as a marginally trapped surface (or simply marginal surface). Penrose's definition is purely local since it involves only quantities defined on the surface $\Sp$.

According to Hawking \cite{Hawking}, an outer trapped surface is an orientable compact spacelike 2-surface $\Sp$ contained in the future development of a partial Cauchy hypersurface $\Sigma_0$ and which is such that the outgoing null geodesics emerging orthogonally from $\Sp$ converge locally at $\Sp$. The definition of outgoing null geodesics is based on the asumption of asymptotic flatness. In the present context, demanding that the spacelike 2-surface $\Sp_t={\cal H}\cap\Sigma_t$ is an outer trapped surface is equivalent to:
\begin{enumerate}[(i)]
	\item the spacelike hypersurface $\Sigma_t$ is asymptotically flat and the scalar field $u$ defining ${\cal H}$ has been chosen so that the exterior or $\Sp_t$ contains the asymptotically flat region, so that \w{$l$} is an outgoing null normal in the sense of Hawking;
	\item the expansion scalar of \w{$l$} is negative or null: $\theta\leq0$.
\end{enumerate}
The subcase $\theta=0$ is referred to as a marginally trapped surface. This definition does not assume anything on $\theta_{\left(k\right)}$.

An apparent horizon was introduced by Hawking \cite{Hawking} and it is defined as a 2-surface ${\cal A}$ inside a Cauchy spacelike hypersurface $\Sigma$ such that ${\cal A}$ is a connected component of the outer boundary of the trapped region of $\Sigma$. By a trapped region, it is meant the set of points of $\Sigma$ through which there is an outer trapped surface lying in $\Sigma$. It can be deduced that an apparent horizon is a marginally outer trapped surface.

We can connect the above definitions with a NEH: if ${\cal H}$ is an NEH in an asymptotically flat spacetime, then each slice $\Sp_t$ is a marginally outer trapped surface. If, in addition, $\theta_{\left(k\right)}\leq0$, then $\Sp_t$ is a marginally trapped surface. In general, \w{$k$} being the inward null normal to $\Sp_t$, $\theta_{\left(k\right)}$ is always negative; however, there exist some pathological situations for which $\theta_{\left(k\right)}>0$ at some points of $\Sp_t$.

\section{Trapping horizons in dynamical spacetimes of BHs: inner boundary conditions}
This Section is based on the Refs.~\cite{CC08, Jaramillo06, CC06, Jaramillo08}. The explicit expressions for the characteristic speeds obtained in Section~\ref{sect:matFCF} are specially useful in the assessment of the boundary conditions to be imposed on a given boundary. This is illustrated by considering inner boundaries in the context of excised black hole spacetimes. Let us point out that FCF can be employed in combination with any of the standard techniques dealing with the black hole singularity in numerical evolutions of black hole spacetimes, namely excision, punctures, moving punctures or stuffed black holes (see next Section). However, the excision technique is favoured if the elliptic subsystem of the FCF is implemented by means of spectral methods; spectral methods are used in elliptic equations with analytical singularities, but it is difficut to treat numerically non-analytical singularities (and also discontinuities) in the (moving) puncture method (see Section \ref{sect:num_treat_BH} for more details).

We are going to consider the problem of inner boundary conditions of trapping horizons of black holes, following Ref.~\cite{Jaramillo06}. We are going to identify a quasi-local horizon as a world tube ${\cal H}$ of apparent horizons, i.e.:
\begin{enumerate}[(i)]
	\item ${\cal H}\approx \mathbb{S}^2\times\mathbb{R}$ is foliated by marginally trapped 2-surfaces ($\theta=0$ and $\theta_{\left(k\right)}<0$);
	\item the condition of future outer trapping horizon, $\Liec{k}\theta_{\left(l\right)}<0$, has to be verified;
	\item the condition of dynamical horizon (DH), ${\cal H}$ is spacelike, has to be verified.
\end{enumerate}


Given a DH ${\cal H}$, the foliation by marginally trapped surfaces is unique, and it defines a unique vector $\w{h}$, which can be written as $\w{h}=N\w{n}+b\w{s}$ (see \cite{Jaramillo06}). ${\cal H}$ is spacelike as long as $\w{h}$ be spacelike, i.e., $b-N>0$.

A coordinate system adapted to the horizon is one such that \w{$t$} is tangent to ${\cal H}$. In a coordinate system all the spheres $\Sp_t$ stay at the same coordinate position, say $r=\mathrm{const}=r_0$. If we write the decomposition of the shift vector with respect to \w{$s$} as $\w{\beta}= \beta^{\bot}\w{s}-\w{V}$, the condition of \w{$t$} tangent to ${\cal H}$ means $\beta^{\bot}=b$; in this case, $\w{h}$ spacelike means $\beta^{\bot}-N>0$.

The previous analysis of the evolution system for $h^{ij}$ can be applied to the inner boundary conditions problem in an excised approach to black hole evolutions. A crucial point in such an approach to black hole evolution is to assess the freedom to impose boundary conditions on the excised surface. To this aim we must determine the characteristics on the excised surface.

We now specify the generic vector $\zeta^i$ as the unitary outgoing radial vector on the horizon, $s_i$. By definition $\beta^{\bot}=\beta^{\mu}s_{\mu}$, so the expressions of the eigenvalues associated to (\ref{e:sisth1}) which are not identical to zero are just $\lambda_{\pm}^{\left(\zeta\right)}=-\beta^{\bot} \pm N$. Because of the conditions mentioned before, that are linked with the boundary conditions of the elliptic equations, we have $-\beta^{\bot} + N < 0$ on the excised surface (which coincides with the black hole horizon). Since the lapse function is positive, then $-\beta^{\bot} - N < 0$. This shows that the characteristics on the excised surface associated with the vector $s^i$ points outwards with respect to the integration domain. There is a key interplay between the elliptic boundary conditions and the properties of the hyperbolic degrees of freedom. All the equations, elliptic and hyperbolic ones, must be considered as a whole strongly coupled system.

The fact that all the characteristic curves are ingoing into the black hole (or outgoing with respect to the integration domain) is something we could expect from the physical intuition. In consequence, there is no residual freedom in the prescription of the inner boundary conditions of $h^{ij}$ during the evolution. The system is fully determined and we must only guarantee that the values of $h^{ij}$ are consistent with the choice of the Dirac gauge (something that can actually be tricky in the numerical implementation).

Of course, it is not obvious how to choose dynamically an inner boundary ${\cal H}$ that is guaranteed to be spacelike during the evolution. One can adopt a coordinate system in order to guarantee ${\cal H}$ to be spacelike and the characteristics are still outgoing from the integration domain (see \cite{CC08} for more details).

